Computational Two-Party Correlation: A Dichotomy for Key-Agreement Protocols

Let $\pi$ be an efficient two-party protocol that given security parameter $\kappa$, both parties output single bits $X_\kappa$ and $Y_\kappa$, respectively. We are interested in how $(X_\kappa,Y_\kappa)$ "appears" to an efficient adversary that only views the transcript $T_\kappa$. We make the following contributions: $\bullet$ We develop new tools to argue about this loose notion and show (modulo some caveats) that for every such protocol $\pi$, there exists an efficient simulator such that the following holds: on input $T_\kappa$, the simulator outputs a pair $(X'_\kappa ,Y'_\kappa)$ such that $(X'_\kappa,Y'_\kappa,T_\kappa)$ is (somewhat) computationally indistinguishable from $(X_\kappa,Y_\kappa,T_\kappa)$. $\bullet$ We use these tools to prove the following dichotomy theorem: every such protocol $\pi$ is: - either uncorrelated -- it is (somewhat) indistinguishable from an efficient protocol whose parties interact to produce $T_\kappa$, but then choose their outputs independently from some product distribution (that is determined in poly-time from $T_\kappa$), - or, the protocol implies a key-agreement protocol (for infinitely many $\kappa$'s). Uncorrelated protocols are uninteresting from a cryptographic viewpoint, as the correlation between outputs is (computationally) trivial. Our dichotomy shows that every protocol is either completely uninteresting or implies key-agreement. $\bullet$ We use the above dichotomy to make progress on open problems on minimal cryptographic assumptions required for differentially private mechanisms for the XOR function. $\bullet$ A subsequent work of Haitner et al. uses the above dichotomy to makes progress on a longstanding open question regarding the complexity of fair two-party coin-flipping protocols.

==> Distinguisher.tex <==
\section{Proof of  \cref{thm:3}}\label{sec:jad}

In this section, we prove \cref{thm:3}. Throughout this section we are dealing with a fixed input length, a fixed deterministic forecaster $\Fc$, and a fixed function $D$. Therefore, to avoid clutter, we will use the term ``forecaster'' rather than ``deterministic forecaster''. We will also make use of the following notation:




\begin{algorithm}[$\Fc'$]\label{fig:From distinguishing to better forecasting}$\mbox{}$
	
	\begin{description}
		\item [Parameters:] Security parameter $1^\secParam$ and  $\gamma,\alpha,\lambda,\rho>0$.
		\item[Input:] $z=(t,r) \in\zo^{m(\kappa)+l(\kappa)}$ and $r'\in\zo^{l'(\kappa)}$.  
		\item [Oracles:] Protocol $\Pi$, triplet $\gamma$-forecaster $\Fc$ and ``distinguisher" $\Dc$.
		\item[Operation:] $\mbox{}$
		\begin{enumerate}
			\item Compute $p=(p_1,p_2,p_3)\from \Fc_\secParam(z)$. 
			\item If one of the following hold:
			\begin{itemize}
				\item $\lambda \le p_1\le1-\lambda$ and $|p_2-p_3|>\lambda$,
				\item $p_1<\lambda$ and $p_2\in([0,\lambda]\cup[1-\lambda,1])$,
				\item $p_1>1-\lambda$ and $p_3\in([0,\lambda]\cup[1-\lambda,1])$,
			\end{itemize}
			then output $p$. 
			\item Set $l=\secParam^3$, $q=(1-p_1)\cdot p_2+p_1\cdot p_3$.
			\item Sample all the following:
				\begin{itemize}
					\item $l=\secParam^3$ independent triplets $(x_1,y_1,z_1)\cdots (x_l,y_l,z_l)$ using $\Pi_\secParam$,
					\item $l$ independent $r_{1}'\cdots r_{l}'$, and
					\item one bit $b\from U_q$ (where $b\from U_q$ is an independent bit with bias $q$).
				\end{itemize}
		%	\item Sample $l=\secParam^3$ independent triplets $(x_1,y_1,z_1)\cdots (x_l,y_l,z_l)$ using $\Pi_\secParam$, and $l$ independent $r_{1}'\cdots r_{l}'$ as randomness for the distinguisher.
			\item Set $I_0={\set{i\colon \Fc_\secParam(z_i)=p\cap x_i=0}}$, $I_1={\set{i\colon \Fc_\secParam(z_i)=p\cap x_i=1}}$ and $I=I_0\cup I_1$.
			\item If $\alpha/2 >\frac{\size{I}}{l}$,  output $p$.
			\item Calculate all the following:
			\begin{itemize}
				\item$d=\frac{\size{\set{i\in I\colon  \Dc_\secParam(x_i,y_i,z_i,r_{i}')=1}}}{\size{I}}$, 
				\item$d_{x}=(1-q)\cdot\frac{\size{\set{i\in I\colon  \Dc_\secParam(x_i,0,z_i,r_{i}')=1}}}{\size{I}} +  q\cdot \frac{\size{\set{i\in I\colon   \Dc_\secParam(x_i,1,z_i,r_{i}')=1}}}{\size{I}}$, 
				\item $d_{y_0}=\frac{\size{\set{i\in I_0\colon  \Dc_\secParam(0,y_i,z_i,r_{i}')=1}}}{\size{I_0}}$ and 
					 $d_{y_1}=\frac{\size{\set{i\in I_1\colon  \Dc_\secParam(1,y_i,z_i,r_{i}')=1}}}{\size{I_1}}$.
			\end{itemize} 
		%	$d=\frac{\size{\set{i\in I\colon  \Dc_\secParam(x_i,y_i,z_i,r_{i}')=1}}}{\size{I}}$, 
		%	$d_{x_0}=\frac{\size{\set{i\in I\colon  \Dc_\secParam(x_i,0,z_i,r_{i}')=1}}}{\size{I}}$,  
		%	$d_{x_1}=\frac{\size{\set{i\in I\colon   \Dc_\secParam(x_i,1,z_i,r_{i}')=1}}}{\size{I}}$, 
		%	$d_{y_0}=\frac{\size{\set{i\in I_0\colon  \Dc_\secParam(0,y_i,z_i,r_{i}')=1}}}{\size{I_0}}$ and 
		%	$d_{y_1}=\frac{\size{\set{i\in I_1\colon  \Dc_\secParam(1,y_i,z_i,r_{i}')=1}}}{\size{I_1}}$.
			%	\item  $d_{y_0}=\frac{\size{\set{i\colon i\in I_0 \cap \Dc_\secParam(0,y_i,z_i)=1}}}{\size{I_0}}$ and $d_{y_1}=\frac{\size{\set{i\colon i\in I_1 \cap \Dc_\secParam(1,y_i,z_i)=1}}}{\size{I_1}}$.
			%	\item   calculate $d_{x_0}=\frac{\size{\set{i\colon i\in I \cap \Dc_\secParam(x_i,0,z_i)=1}}}{\size{I}}$ and $d_{x_1}=\frac{\size{\set{i\colon i\in I \cap \Dc_\secParam(x_i,1,z_i)=1}}}{\size{I}}$.
			
			%	$d_0=\frac{\size{\set{i\colon i\in I_0 \cap \Dc_\secParam(0,y_i,z_i)=1}}}{\size{I_0}}$ and $d_1=\frac{\size{\set{i\colon i\in I_1 \cap \Dc_\secParam(1,y_i,z_i)=1}}}{\size{I_1}}$.
			\item $(d',d_{y_0}',d_{y_1}')\from \Help(p)$.
			
			\item If $|d-d'|<\rho/10$ then output $p$.
			\item If $d-d'\ge \rho/10$ set $s=1$ otherwise set $s=-1$.
			\item Set $(p_{1}',p_{2}',p_{3}')=(p_{1},p_{2},p_{3})$, and consider the following cases:
			\begin{description}						
				\item [Case 1:] If  $\lambda<p_1<1-\lambda$ and $s(d_{x}-d')>\rho/50$ and $\Dc_\pk(1,b,z,r')\neq \Dc_\pk(0,b,z,r')$  then set $p_{1}'=p_1 +  s\cdot\gamma\cdot (2\Dc_\pk(1,b,z,r')-1)$.  
			%	\item [Case 2:] If  $\lambda<p_1<1-\lambda$ and $s(d_{x_1}-d_{x_1}')>\rho/50$ and $\Dc_\pk(1,1,z,r')\neq \Dc_\pk(0,1,z,r')$  then set $p_{1}'=p_1 + s\cdot\gamma\cdot (2\Dc_\pk(1,1,z,r')-1)$.
				
				\item [Case 2:] If  $p_1<1-\lambda$ and $s(d_{y_0}-d_{y_0}')>\rho/50$ and $\Dc_\secParam(0,1,z,r')\neq \Dc_\pk(0,0,z,r')$  then set $p_{2}'=p_2 + s\cdot\gamma\cdot (2\Dc_\pk(0,1,z,r')-1)$.
				\item [Case 3:] If  $p_1>\lambda$ and $s(d_{y_1}-d_{y_1}')>\rho/50$ and $\Dc_\pk(1,1,z,r')\neq \Dc_\pk(1,0,z,r')$  then set $p_{3}'=p_3 + s\cdot\gamma\cdot (2\Dc_\pk(1,1,z,r')-1)$.
			\end{description}
			
			
			\item Output $(p_{1}',p_{2}',p_{3}')$.
		\end{enumerate}
	\end{description}
	
\end{algorithm}


\begin{algorithm} [\Help:]   \label{fig:Distinguishing on atom}$\mbox{}$
	\begin{description}
		\item [Parameters:] Security parameter $1^\secParam$ and  $\gamma,\alpha,\lambda,\rho>0$.
		\item[Input:] An atom $p=(p_1,p_2,p_3)$ and $r'\in\zo^{l'(\kappa)}$.
		\item [Oracles:] protocol $\Pi$, triplet $\gamma$-forecaster $\Fc$ and ``distinguisher" $\Dc$.
		\item[Operation:] $\mbox{}$
		\begin{enumerate}
			\item Calculate $q=(1-p_1)\cdot p_2+p_1\cdot p_3$.
			\item Sample $l=\secParam^3$ independent triplets $(x_1,y_1,z_1)\cdots (x_l,y_l,z_l)$ using $\Pi_\secParam$.
			\item Set $I_0={\set{i\colon \Fc_\secParam(z_i)=p\cap x_i=0}}$ and $I_1={\set{i\colon \Fc_\secParam(z_i)=p\cap x_i=1}}$ and $I=I_0\cup I_1$. 
			\item Sample $l$ independent pairs $(b_{1}^x,b_{1}^y)\cdots (b_{l}^x,b_{l}^y)$ from $(U_{p_1},U_q)$, (where $b\from U_q$ is an independent bit with bias $q$).   
			\item For every $i\in l$ we define a new triplet $(b_{i}^x,b_{i}^y,z_i)$ by replacing $(x_i,y_i)$ with $(b_{i}^x,b_{i}^y)$.
			\item Calculate all the following:
		$d=\frac{\size{\set{i\in I\colon  \Dc_\secParam(b_{i}^x,b_{i}^y,z_i,r')=1}}}{\size{I}}$, 
	%	\item	$d_{x}=(1-q)\frac{\size{\set{i\in I\colon  \Dc_\secParam(b_{i}^x,0,z_i,r')=1}}}{\size{I}}$,  
	%		$d_{x_1}=\frac{\size{\set{i\in I\colon  \Dc_\secParam(b_{i}^x,1,z_i,r')=1}}}{\size{I}}$, 
		$d_{y_0}=\frac{\size{\set{i\in I_0\colon \Dc_\secParam(0,b_{i}^y,z_i,r')=1}}}{\size{I_0}}$ and 
			$d_{y_1}=\frac{\size{\set{i\in I_1\colon \Dc_\secParam(1,b_{i}^y,z_i,r')=1}}}{\size{I_1}}$.
	
			\item Output $(d,d_{y_0},d_{y_1})$.
			
		\end{enumerate}
	\end{description}
\end{algorithm}







\begin{definition}[distributions]\label{def:distributions}
	Let $n$ be a parameter, we make the following definitions
	\begin{itemize}
		\item We say that $(X,Y,T)$ are a triplet, if $(X,Y,T)$ are distributed together over $\zo\times\zo\times\zn$,
		\item and say that $(X,T)$ are a  pair, if $(X,T)$ are distributed together over $\zo\times\zn$.
	\end{itemize}
\end{definition}

\begin{definition}[conditional price]
	Let $Z=(X,T)$ denote a pair and let $\Fc$ be a $\fpartial$ $\gamma$-\forecaster. Let $B$ be an event, we define the conditional price of $\Fc$ with respect to $Z$ as follows:
	$$
	\Price_Z(\Fc|B)=\Price_{Z|B}(\Fc)
	$$ 
\end{definition}

Theorem \ref{thm:3} follows from the following lemma (which is the main lemma of this section) by choosing $\nu=\lambda$.

\begin{lemma}\label{lemma:Distinguishing to better forecasting}
	Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ be a $\gamma$-$\forecaster$. Let $\Fc_{1},\Fc_{2},\Fc_{3}$ denote the three $\fpartial$	$\gamma$-$\forecaster$ such that for every $t\in \zn$, $\Fc(t)=(\Fc_{1}(t),\Fc_{2}(t),\Fc_{3}(t))$ and define the following events: $G_0=\set{\Fc_1(T)\le\nu}$, $G_1=\set{\Fc_1(T)\ge 1-\nu}$ and $G_2=\set{|\Fc(T)_2-\Fc(T)_3|<\lambda}$. Let $\Dc:\zo\times\zo\times\zn\to\zo$   be a function and defined the functions $\Fc_x$, $\Fc_y$ as follows: for every $t\in \zn$, $\Fc_x(t)=\Fc_1(t)$ and $\Fc_y(t)=(1-\Fc_1(t))\Fc_2(t)+\Fc_1(t)\Fc_3(t)$. If
	\begin{enumerate}
		\item $\pr{G_0\cup G_1\cup G_2}>1-\beta$ and
		\item $\pr{\Dc(X,Y,T)=1}-\pr{\Dc(U_{\Fc_x(T)},U_{\Fc_y(T)},T)=1}>\rho$, where $\rho>10\nu+300\sqrt{\gamma}+3\lambda +\beta$ and $\lambda,\nu\ge 1000\sqrt{\gamma}$ .
	\end{enumerate}
	Then there exists a $\gamma$-$\forecaster$ $\Fc^\ast$ (which can be constructed in $\poly$-time given access to $\Fc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)\ge \mu $, for $\mu=\gamma^8$.
\end{lemma}

The remainder of this section is devoted to proving Lemma \ref{lemma:Distinguishing to better forecasting}.
Our first step will be to develop machinery for partial forecasters (which we will later use when we handle forecasters that output three numbers).
We will prove the following lemma (which can be thought of as a version of Lemma \ref{lemma:Distinguishing to better forecasting} for the case of partial forecasters).

\begin{lemma}\label{lemma:Partial forecaster distinguishing}
	Let $Z=(X,T)$ denote a pair (that can be sampled in poly-time by an algorithm). Let $\nu,q$ be constants such that $q\in\cW_\gamma$ and $\nu\le q \le 1-\nu$ , and let $\Fc$ be a $\fpartial$ $\gamma$-\forecaster such that for every $t\in \Supp(T)$, $\Fc(t)=q$. Let $\Dc: \zo\times\zn\to\zo$ be a function such that $\pr{\Dc(X,T)=1}-\pr{\Dc(U_{\Fc(T) },T)=1}>\rho,$
	then there exists a $\fpartial$ $\gamma$-\forecaster $\Fc^\ast$ (which can be constructed in $\poly$-time given access to $\Fc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)>\mu$, for $\mu=\gamma(2\rho-\gamma)$.
\end{lemma}

This section is arranged as follows: In Section \ref{sec:jad:partial} we prove Lemma \ref{lemma:Partial forecaster distinguishing}. In Section \ref{sec:jad:full} we prove Lemma \ref{lemma:Distinguishing to better forecasting}.


\subsection{Partial Forecaster Distinguishing}
\label{sec:jad:partial}

%\jnote{Here I am assuming that $\Dc$ the distinguisher is deterministic, I am not quite sure how to define things correctly, so I am leaving this for now, but this should be dealt with.}\\
%\Jnote{I also assume that $q$ that is chosen is not $0$ or $1$, It's not a problem but I forgot to deal with it}

In this section we prove Lemma \ref{lemma:Partial forecaster distinguishing}.
We consider the following algorithm (that is used to update an estimate $q$ of a forecaster) using a ``distinguisher''.

\begin{algorithm}[$\Fc^\ast$ the improved forecaster]\label{alg:improved forecaster}
	\item[Parameter:] $\gamma>0$ and $q \in \cW_\gamma$, such that $\nu<q<1-\nu$.
	\item[Oracles:] function $\Dc$.
	\item [Input:] $t\in \zn$
	\begin{enumerate}
		\item If $\Dc(1,t)=1$ output $(q+\gamma)$
		\item If $\Dc(1,t)=0$ output $(q-\gamma)$	
	\end{enumerate}
\end{algorithm}




\begin{claim}\label{claim:partial forecaster Cal}	
	Let $Z=(X,T)$ be a pair, let $q\in\cW_\gamma$ be a constant. Let $\Fc$ be a $\fpartial$ $\gamma$-\forecaster and let $\Dc: \zo\times\zn\to\zo$ be a function such that for every $t\in \Supp(T)$, $\Fc(t)=q$ and, $\Dc(1,t)\ne \Dc(0,t)$. Then we have that
	\[\pr{\Dc(X,T)=1}-\pr{\Dc(U_{q},T)=1}=\pr{X=1}((1-q)\cdot(2\alpha_1-1))+\pr{X=0}(q\cdot(2\alpha_0 -1)),\]
	where we define $\alpha_0=\pr{\Dc(0,T)=1|X=0}$ and $\alpha_1=\pr{\Dc(1,T)=1|X=1}$.
\end{claim}
\begin{proof}
	It is clear that $\pr{\Dc(X,T)=1}= \pr{X=1}\cdot\alpha_1+\pr{X=0}\cdot\alpha_0$, on the other hand,
	\begin{align*}
	\pr{\Dc(U_{q},T)=1}&=\pr{X=1}\cdot\pr{\Dc(U_{q},T)=1|X=1}+\pr{X=0}\cdot\pr{\Dc(U_{q},T)=1|X=0}\\
	&=\pr{X=1}(\pr{\Dc(1,T)=1|X=1}\cdot q+\pr{\Dc(0,T)=1|X=1}\cdot(1-q))\\
	&+\pr{X=0}(\pr{\Dc(1,T)=1|X=0}\cdot q+\pr{\Dc(0,T)=1|X=0}\cdot(1-q))		
	\end{align*}
	Since $\Dc(1,t)\ne \Dc(0,t)$ for every $t\in \Supp(T)$, we have $1-\alpha_0=\pr{\Dc(1,T)=1|X=0}$ and $1-\alpha_1=\pr{\Dc(0,T)=1|X=1}$. Thus we get that
	$$
	\pr{\Dc(U_{q},T)=1}=\pr{X=1}(q\cdot\alpha_1+(1-q)\cdot(1-\alpha_1))+\pr{X=0}(q\cdot(1-\alpha_0)+(1-q)\cdot\alpha_0)	
	$$
	putting the two together,
	\begin{align*}
	\pr{\Dc(X,T)=1}-\pr{\Dc(U_{q},T)=1}&=\pr{X=1}((1-q)\alpha_1-(1-q)(1-\alpha_1))+\pr{X=0}(q\alpha_0 -q(1-\alpha_0))\\
	&=\pr{X=1}((1-q)\cdot(2\alpha_1-1))+\pr{X=0}(q\cdot(2\alpha_0 -1))	
	\end{align*}
	as desired.
\end{proof}



\begin{lemma}\label{lemma:Improved partial forecaster value}
	
	Let $Z=(X,T)$ be a pair that can be sampled in poly-time, and let $q,\nu>0$  be constants such that $q\in\cW_\gamma$, $\nu \le q \le 1-\nu$. Let $\Fc$ be a $\fpartial$ $\gamma$-\forecaster and let $\Dc: \zo\times\zn\to\zo$ be a function such that for every $t\in \Supp(T)$, $\Fc(t)=q$ and $\Dc(1,t)\ne \Dc(0,t)$. Define the $\fpartial$ $\gamma$-\forecaster $\Fc^\ast$ as described in Algorithm \ref{alg:improved forecaster} using $q$, $\Fc$ and $\Dc$. We have that:
	\[\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast) =\gamma\bigg(2\Big(\pr{X=1}\big((1-q)(2\alpha_1-1)\big)+\pr{X=0}\big(q(2\alpha_0-1)\big)\Big)-\gamma\bigg) \]
	where we define $\alpha_0=\pr{\Dc(0,T)=1|X=0}$ and $\alpha_1=\pr{\Dc(1,T)=1|X=1}$.
\end{lemma}
\begin{proof}
	The proof will proceed in two steps, we first calculate the difference in the price function for the case where $X=1$ and then for the case where $X=0$, as stated in the following two claims:
	\begin{claim}
		$\Price_{Z}(\Fc|X=1)-\Price_{Z}(\Fc^\ast|X=1) =\gamma(2(1-q)(2\alpha_1-1)-\gamma)$
	\end{claim}
	\begin{proof}
		We have that
		\begin{align*}
		\Price_{Z}(\Fc|X=1)-&\Price_{Z}(\Fc^\ast|X=1)=\\
		&+\pr{\Dc(1,T)=1|X=1}\cdot \big(\Price_{Z}(\Fc|\Dc(1,T)=1,X=1)-\Price_{Z}(\Fc^\ast|\Dc(1,T)=1,X=1) \big)\\
		&+\pr{\Dc(1,T)=0|X=1}\cdot \big(\Price_{Z}(\Fc|\Dc(1,T)=0,X=1)-\Price_{Z}(\Fc^\ast|\Dc(1,T)=0,X=1) \big)
		\end{align*}
		First note that by definition	
		$$
		\Price_{Z}(\Fc|X=1)=\Price_{Z}(\Fc|\set{\Dc(1,T)=1,X=1})=\Price_{Z}(\Fc|\set{\Dc(1,T)=0,X=1})=(1-q)^2,
		$$
		since the output of $\Fc$ does not depend on $\Dc$. But $\Fc^\ast$ is defined using $\Dc$, such that for every $t\in \Supp(T)$, if $\Dc(1,t)=1$ then $\Fc^\ast(t)$ will output $q+\gamma$, otherwise it outputs $q-\gamma$.
		Thus we get that
		\[\Price_{Z}(\Fc^\ast|\set{\Dc(1,T)=1,X=1})=(1-(q+\gamma))^2= (1-q)^2 -2\gamma(1-q)+\gamma^2\]
		\[\Price_{Z}(\Fc^\ast|\set{\Dc(1,T)=0,X=1})=(1-(q-\gamma))^2= (1-q)^2 +2\gamma(1-q)+\gamma^2\]
		Putting the two together we get that
		\begin{itemize}
			\item $\Price_{Z}(\Fc|\set{\Dc(1,T)=1,X=1})-\Price_{Z}(\Fc^\ast|\set{\Dc(1,T)=1,X=1})= +2\gamma(1-q)-\gamma^2$
			\item $\Price_{Z}(\Fc|\set{\Dc(1,T)=0,X=1})-\Price_{Z}(\Fc^\ast|\set{\Dc(1,T)=0,X=1})= -2\gamma(1-q)-\gamma^2$
		\end{itemize}	
		Recall that $\alpha_1=\pr{\Dc(1,T)=1|X=1}$ and $1-\alpha_1=\pr{\Dc(1,T)=0|X=1}$, thus we get that
		\begin{align*}
		\Price_{Z}(\Fc|X=1)-\Price_{Z}(\Fc^\ast|X=1)&=\alpha_1\cdot(2\gamma(1-q)-\gamma^2)+(1-\alpha_1)\cdot(-2\gamma(1-q)-\gamma^2)\\
		&=\alpha_1\cdot(2\gamma(1-q))+(1-\alpha_1)\cdot(-2\gamma(1-q))-\gamma^2\\
		&=2\gamma(1-q)(2\alpha_1-1)	-\gamma^2
		\end{align*}
		as desired
	\end{proof}
	Similarly we will now show that
	
	\begin{claim}
		$\Price_{Z}(\Fc|X=0)-\Price_{Z}(\Fc^\ast|X=0) =\gamma(2q(2\alpha_0-1)-\gamma)$
	\end{claim}
	\begin{proof}
		We have that
		\begin{align*}
		\Price_{Z}(\Fc|X=0)-&\Price_{Z}(\Fc^\ast|X=0)=\\
		&+\pr{\Dc(1,T)=1|X=0}\cdot \big(\Price_{Z}(\Fc|\Dc(1,T)=1,X=0)-\Price_{Z}(\Fc^\ast|\Dc(1,T)=1,X=0) \big)\\
		&+\pr{\Dc(1,T)=0|X=0}\cdot \big(\Price_{Z}(\Fc|\Dc(1,T)=0,X=0)-\Price_{Z}(\Fc^\ast|\Dc(1,T)=0,X=0) \big)
		\end{align*}
		Note that by definition	
		$$
		\Price_{Z}(\Fc|X=0)=\Price_{Z}(\Fc|\set{\Dc(1,T)=1,X=0})=\Price_{Z}(\Fc|\set{\Dc(1,T)=0,X=0})=q^2,
		$$
		since the output of $\Fc$ does not depend on $\Dc$. But $\Fc^\ast$ is defined using $\Dc$, such that for every $t\in \Supp(T)$, if $\Dc(1,t)=1$ then $\Fc^\ast(t)$ will output $q+\gamma$, otherwise it outputs $q-\gamma$.
		Thus we get that 	
		\[\Price_{Z}(\Fc^\ast|\set{\Dc(1,T)=1,X=0})=(q+\gamma)^2= q^2 +2q\gamma +\gamma^2\]
		\[\Price_{Z}(\Fc^\ast|\set{\Dc(1,T)=0,X=0})=(q-\gamma)^2= q^2 -2q\gamma+\gamma^2\]
		Putting the two together we get that
		\begin{itemize}
			\item $\Price_{Z}(\Fc|\set{\Dc(1,T)=1,X=0})-\Price_{Z}(\Fc^\ast|\set{\Dc(1,T)=1,X=0})= -2q\gamma-\gamma^2$
			\item $\Price_{Z}(\Fc|\set{\Dc(1,T)=0,X=0})-\Price_{Z}(\Fc^\ast|\set{\Dc(1,T)=0,X=0})= +2q\gamma-\gamma^2$
		\end{itemize}	
		Recall that $\alpha_0=\pr{\Dc(0,T)=1|X=0}$ and since $\Dc(1,t)\ne \Dc(0,t)$ for every $t\in \Supp(T)$, we have $\alpha_0=\pr{\Dc(1,T)=0|X=0}$ and $1-\alpha_0=\pr{\Dc(1,T)=1|X=0}$. %\jnote{Someone else should also check that I didn't cheat here.} 
		We get that
		\begin{align*}
		\Price_{Z}(\Fc|X=0)-\Price_{Z}(\Fc^\ast|X=0)&=\alpha_0\cdot(2q\gamma -\gamma^2)+(1-\alpha_0)\cdot(-2q\gamma-\gamma^2)\\
		&=\alpha_0\cdot(2q\gamma)+(1-\alpha_0)\cdot(-2q\gamma)-\gamma^2\\
		&=2q\gamma(2\alpha_0-1)	-\gamma^2
		\end{align*}
		and the claim hold.
	\end{proof}	
	By using the above two claims, and by that fact that
	\begin{align*}
	\Price_{Z}&(\Fc)-\Price_{Z}(\Fc^\ast)=\\
	&+\pr{X=1}\cdot(\Price_{Z}(\Fc|X=1)-\Price_{Z}(\Fc^\ast|X=1))+\pr{X=0}\cdot (\Price_{Z}(\Fc|X=0)-\Price_{Z}(\Fc^\ast|X=0)).
	\end{align*}
	The lemma holds.
\end{proof}


We are now ready to prove Lemma \ref{lemma:Partial forecaster distinguishing}.


\begin{proof} (of Lemma \ref{lemma:Partial forecaster distinguishing}
	Let $G$ denote the set of  "transcripts" such that $G=\set{t\colon\Dc(1,t)\ne\Dc(0,t)}$. It is easy to see that $\pr{\Dc(X,T)=1|T\notin G}-\pr{\Dc(U_{\Fc(T)},T)=1|T\notin G} =0,$
	since in this case $\Dc$ is essentially a function of $T$. Thus we get that:
	\begin{align*}
	\pr{\Dc(X,T)=1}-\pr{\Dc(U_{q},T)=1} &=\pr{T\in G}\cdot(\pr{\Dc(X,T)=1|T\in G}-\pr{\Dc(U_{q},T)=1|T\in G})
	\end{align*}
	Let $\rho'=\pr{\Dc(X,T)=1|T\in G}-\pr{\Dc(U_{q},T)=1|T\in G}$, we get that $\pr{T\in G}>\frac{\rho}{\rho'}$ and  $\rho'>\rho$.
	We can now define the pair $Z'=(X',T')=((X,T)|\set{T\in G})$\footnote{Z' can still be sampled since $\rho<\pr{T\in G}$ and $\Dc$ runs in poly-time.} and we make the following notation  $\alpha_0=\pr{\Dc(0,T')=1|X'=0}$ and $\alpha_1=\pr{\Dc(1,T')=1|X'=1}$. Note that for every $t'\in T'$ we have that $\Dc(1,t')\ne\Dc(0,t')$ and so by Claim \ref{claim:partial forecaster Cal} we get that
	\[\rho'=\pr{\Dc(X',T')=1}-\pr{\Dc(U_{q},T')=1}=\pr{X'=1}((1-q)\cdot(2\alpha_1-1))+\pr{X'=0}(q\cdot(2\alpha_0 -1)),\]
	and since by assumption we also have that $\nu\le q \le 1-\nu$, we can define the $\fpartial$ $\gamma$-\forecaster $\Fc'$ as described in Algorithm \ref{alg:improved forecaster} for $q$ and $\Dc$. By Lemma \ref{lemma:Improved partial forecaster value} we get that:
	\begin{align*}
	\Price_{Z'}(\Fc)-\Price_{Z'}(\Fc') &=\gamma\bigg(2\Big(\pr{X'=1}\big((1-q)(2\alpha_1-1)\big)+\pr{X'=0}\big(q(2\alpha_0-1)\big)\Big)-\gamma\bigg)\\
	&= \gamma(2\rho' -\gamma).
	\end{align*}
	
	% We get that there exists  $\Fc'$ a $\fpartial$ $\gamma$-\forecaster for  $T'$ such that $\Price_{Z'}(\Fc)-\Price_{Z'}(\Fc') = \gamma(2\rho' -\gamma)$.\\
	Using $\Fc'$ we can define the  $\fpartial$ $\gamma$-\forecaster $\Fc^\ast$ this time for $T$ (not $T'$). For every $t\in \Supp(T)$:
	\[\Fc^\ast(t)= \left\{ \begin{array}{ll}
	\Fc'(t) & \mbox{if } t\in G \\
	\Fc(t) & \mbox{otherwise }
	\end{array} \right. \]       	
	Thus we get that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)= (\Price_{Z'}(\Fc)-\Price_{Z'}(\Fc'))\cdot \pr{T\in G}= \gamma(2\rho'-\gamma)\pr{T\in G}> \gamma(2\rho-\gamma)$ and the claim holds.
\end{proof}


\subsection{Distinguishing  to Forecasting}
\label{sec:jad:full}

%\begin{theorem}\label{Thm:no correlation implies indistinguishability}
%	Let $Z=(X,Y,T)$ be a triplet such that $\pr{X=1}\notin{\zo}$,\footnote{This is something we will have to deal with later as an independent case, but to make things full defined we have to add this assumption.} and let $\Fc$ be a $\full$ $\gamma$-$\forecaster$ for $T$ that is $(\gamma^8)$-\minimal with respect to $Z$. If
%	\[\pr{|\Fc(T)_2-\Fc(T)_3|<\lambda}\geq 1-\beta \]
%	then $(X,Y,T)$ is computationally $(2\gamma+\lambda+\beta)$-indistinguishable
%	%\footnote{$\rho$ must be larger that $\gamma$, we chose it to be $2\gamma$ and everything should be fine, we chose $\mu$ the minimality accordingly.}
%	from $(U_{\Fc_x(T)},U_{\Fc_y(T)},T)$, where for every $t \in \Supp(T)$ we define $\Fc_x(t)=\Fc(t)_1$ and $\Fc_y(t)=\frac{\Fc(t)_2+\Fc(t)_3}{2}$.
%\end{theorem}
%\begin{proof}
%	Assume for contradiction that this does not hold. Then there exists a function $\Dc:\zo\times\zo\times\zn\to\zo$ such that
%	\[ \pr{\Dc(X,Y,T)=1}-\pr{\Dc(U_{\Fc_x(T)},U_{\Fc_y(T)},T)=1}\geq  2\gamma+\lambda+\beta \]
%	 and by lemma \ref{lemma:distinguisher to better forecaster}, this means that there exists $\Fc^\ast$ a $\full$ $\gamma$-$\forecaster$ such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)>(1-\beta)\cdot\frac{1}{2}\gamma^6\cdot(\gamma-2\gamma^4)>\gamma^8$  (for any logical choice of $\beta$) contradicting the minimality of $\Fc$.
%\end{proof}





In this section we prove Lemma \ref{lemma:Distinguishing to better forecasting}.
We will first state and prove the following claims and lemmas.




\begin{claim}
	Let $(V,T)$ be a pair (that can be sampled in poly-time) and let $a,\nu\ge0$ be constants such that $a\in\zo$. If $\pr{V=a}\ge 1-\nu$ then the pairs $(V,T)$ and $(a,T)$ are $\nu$ statistically close.
\end{claim}
\begin{proof}
	Assume for contradiction that the claim does not hold. This means that there exists a function $D:\zo\times\zn\to\zo$ (computationally unbounded) such that $|\pr{D(V,T)=1}-\pr{D(a,T)=1}|>\nu$.
	 Let $p,\overline{a}$ be constants such that $p=\pr{V=a}$, $\overline{a}\in\zo$ and it holds that $\overline{a}\ne a$, we get that
\begin{align*}
\nu<|\pr{D(V,T)=1}-\pr{D(a,T)=1}|&\le p|(\Pr[D(V,T)=1|V=a]-\Pr[D(a,T)=1|V=a])|\\
&+(1-p)|(\Pr[D(V,T)=1|V=\overline{a}]-\Pr[D(a,T)=1|V=\overline{a}])|\\
&\le (1-p)
\end{align*}
But by definition $(1-p)\le\nu$, and this is a contradiction.
\end{proof}

%\begin{lemma}
%	Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ be a $\full$ $\gamma$-\forecaster for $T$. Let $(q_1,q_2,q_3)\in\cW_{\gamma}^3$ such that, $\pr{\Fc(T)=(q_1,q_2,q_3)}\geq \gamma^5$. We define $Z=(X',Y',T')|\Fc(T)=(q_1,q_2,q_3)$ and the three pairs $Z_1=(V_1,T_1)=(X',T')$,\footnote{we have to make sure that they are well define} $Z_2=(V_2,T_2)=(Y',T')|X'=0$ and $Z_3=(V_3,T_3)=(Y',T')|X'=1$. If at least one of the following holds:
%	\begin{enumerate}
%		\item $\size{\pr{V_1=1}-q_1}>100\sqrt{\gamma}$
%		\item $\pr{X'=1}>\gamma^{10}$ and $\size{\pr{V_2=1}-q_2}>100\sqrt{\gamma}$
%		\item $\pr{X'=0}>\gamma^{10}$ and $\size{\pr{V_3=1}-q_3}>100\sqrt{\gamma}$
%	\end{enumerate}
%	Then there exists $\Fc'$ a $\full$ $\gamma$-$\forecaster$ (that can be constructed in poly-time, given access to $\Fc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc')\geq \pr{\Fc(T)=(q_1,q_2,q_3)}\cdot(\gamma)\geq\gamma^6$.
%\end{lemma}


%\begin{claim}\label{claim:relative atom size}
%	Let $Z=(X,Y,T)$ be a pair (that can be sampled) and let $\Fc$ be a $\full$ $\gamma$-$\forecaster$ for $T$. Let $\nu,q,b_0,b_1$ be constants such that $q,b_0,b_1\in\cW_\gamma$, $pr{\Fc(T)=(q,b_0,b_1)>\gamma^5$, and $\pr{X=a}$, Let $a,\nu$ be a constants such that $a\in\zo$ and $\size{a-q}<\nu$. Then one of the following must hold
%	\begin{enumerate}
%		\item $(V,T)$ is statistically $(2\nu+100\sqrt{\gamma})$-close to $(U_q,T)$.
%		\item There exists $\Fc'$ a $\fpartial$ $\gamma$-$\forecaster$ (that can be constructed in poly-time, given access to $\Fc$) for $T$ such that $\Price_Z(\Fc)-\Price_Z(\Fc')\geq \gamma$.
%	\end{enumerate}
%	We stress out that the claim holds only when the pair $(X,T)$ can be sampled in poly-time.
%\end{claim}


\begin{claim}\label{claim:dist from exp imply better partial forecaster}
Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ to be a $\gamma$-$\forecaster$. Let $q_1,q_2,q_3,\alpha$ be constants such that $w=(q_1,q_2,q_3)\in\cW_{\gamma}^3$, and define the three pairs: $Z_1=(V_1,T_1)=(X,T)$, $Z_{2}=(V_{2},T_{2})=((Y,T)|X=0)$ and $Z_{3}=(V_{3},T_{3})=((Y,T)|X=1)$. For every index $i\in\{1,2,3\}$, if $\pr{\Fc(T_i)=w}>\alpha\ge\gamma^7$ then one of the following holds,
\begin{enumerate}
	\item There exists $\Fc'$ a $\gamma$-$\forecaster$ (that can be constructed in poly-time, given access to $\Fc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc')\geq \gamma\cdot\pr{\Fc(T_i)=w}\ge \gamma\cdot\alpha$.
	\item  $|q_i-\pr{V_i=1|\Fc(T)=w}|< 100\sqrt{\gamma}$
\end{enumerate}
\end{claim}

Claim \ref{claim:dist from exp imply better partial forecaster} follows by a similar argument to the proof of \ref{lem:accuracy partial forecaster}.


%\begin{lemma}
%	Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ be a $\fpartial$ $\gamma$-\forecaster for $T$. Let $w=(q,b_0,b_1)\in\cW_{\gamma}^3$, such that, $\pr{\Fc(T)=(q_1,q_2,q_3)}\geq \gamma^5$. We define the three pairs $Z_1=(V_1,T_1)=(X,T)$, $Z_2=(V_2,T_2)=(Y,T)|X=0$ and $Z_3=(V_3,T_3)=(Y,T)|X=1$. If at least one of the following holds:
%	\begin{enumerate}
%		\item $\size{\pr{V_1=1}-q_1}>100\sqrt{\gamma}$
%		\item $\pr{X'=1}>\gamma^{10}$ and $\size{\pr{V_2=1}-q_2}>100\sqrt{\gamma}$
%		\item $\pr{X'=0}>\gamma^{10}$ and $\size{\pr{V_3=1}-q_3}>100\sqrt{\gamma}$
%	\end{enumerate}
%	Then there exists $\Fc'$ a $\full$ $\gamma$-$\forecaster$ (that can be constructed in poly-time, given access to $\Fc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc')\geq \pr{\Fc(T)=(q_1,q_2,q_3)}\cdot(\gamma)\geq\gamma^6$.
%\end{lemma}



%\begin{claim}\label{claim:pair-resample-SD}
%	Let $Z=(V,T)$ be a pair (that can be sampled in poly-time) and let $\Fc$ be a $\fpartial$ $\gamma$-$\forecaster$ for $T$, such that for every $t\in T$, $\Fc(t)=q$. Let $a,\nu$ be a constants such that $a\in\zo$ and $\size{a-q}<\nu$. Then one of the following must hold
%	\begin{enumerate}
%		\item $(V,T)$ is statistically $(2\nu+100\sqrt{\gamma})$-close to $(U_q,T)$.
%		\item There exists $\Fc'$ a $\fpartial$ $\gamma$-$\forecaster$ (that can be constructed in poly-time, given access to $\Fc$) for $T$ such that $\Price_Z(\Fc)-\Price_Z(\Fc')\geq \gamma$.
%	\end{enumerate}
%	We stress out that the claim holds only when the pair $(X,T)$ can be sampled in poly-time.
%\end{claim}


\begin{claim}\label{claim:triplet-edeg-resample}
	Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ be a $\gamma$-$\forecaster$. Let $q_1,q_2,q_3,a,\nu,\alpha\ge 0$ be constants such that $w=(q_1,q_2,q_3)\in\cW_{\gamma}^3$ and define the three pairs: $Z_1=(V_1,T_1)=(X,T)$, $Z_{2}=(V_{2},T_{2})=((Y,T)|X=0)$ and $Z_{3}=(V_{3},T_{3})=((Y,T)|X=1)$. For every index $i\in\{1,2,3\}$, if $\pr{\Fc(T_i)=w}>\alpha\ge \gamma^7$ and there exists $a\in\zo$ such that $|q_i-a|<\nu$ then one of the following must hold
	\begin{enumerate}
		\item There exists $\Fc'$ a $\gamma$-$\forecaster$ (that can be constructed in poly-time, given access to $\Fc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc')\geq \gamma\cdot\pr{\Fc(T_i)=w}\ge\gamma\alpha$.
		\item $((V_i,T_i)|\Fc(T_i)=w)$ is statistically $(2\nu+100\sqrt{\gamma})$-close to $((U_{q_i},T_i)|\Fc(T_i)=w)$.
	\end{enumerate}
\end{claim}
\begin{proof}
	The proof follows from the above two claims.	
\end{proof}



%\begin{claim}\label{claim:triplet-edeg-resample-for-y}
%	Let $Z=(X,Y,T)$ be a triplet, $\Fc$ to be a $\full$ $\gamma$-$\forecaster$ for $T$ and denote by $\Fc_1,\Fc_2,\Fc_3$ the three $\fpartial$ $\gamma$-$\forecaster$ that compose $\Fc$. Let $q,b_0,b_1,a,\nu$ be constant such $w=(q,b_0,b_1)\in\cW_{\gamma}^3$ and define the three pairs: $Z_1=(V_1,T_1)=(X,T)$, $Z_{2}=(V_{2},T_{2})=((Y,T)|X=0)$ and $Z_{3}=(V_{3},T_{3})=((Y,T)|X=1)$. For every index $i\in\zo$, if $\pr{\Fc(T)=w}>\gamma^5$, $\nu<q<1-\nu$ and there exists $a\in\zo$ such that $|b_i-a|<\nu$ then one of the following must hold
%	\begin{enumerate}
%		\item There exists $\Fc'$ a $\full$ $\gamma$-$\forecaster$ (that can be constructed in poly-time, given access to $\Fc$) for $T$ such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc')\geq \gamma\cdot\pr{\Fc(T_i)=w}$.
%		\item $((V_i,T_i)|\Fc(T)=w)$ is statistically $(3\nu+100\sqrt{\gamma})$-close to $((U_{b_i},T_i)|\Fc(T)=w)$ and $|q-\pr{X=1|\Fc(T)=w}|<100\sqrt{\gamma}$.
%	\end{enumerate}
%\end{claim}


\begin{claim}\label{claim:conditional atoms size}
	Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ be a $\gamma$-$\forecaster$. Let $q,b_0,b_1,a,\alpha\ge 0$ be constants such that $a\in\zo$ and $q,b_0,b_1\in\cW_\gamma$. Define the tree pairs $Z_x=(V_x,T_x)=(X,T)$, $Z_{y_0}=(V_{y_0},T_{y_0})=((Y,T)|X=0)$ and $Z_{y_1}=(V_{y_1},T_{y_1})=((Y,T)|X=1)$. If $\Pr[\Fc(T)=(q,b_0,b_1)]\ge\gamma^5$ and $\pr{X=a|\Fc(T)=(q,b_0,b_1)}\ge\alpha$ then $\Pr[\Fc(T_{y_a})=(q,b_0,b_1)]\ge\gamma^5\cdot\alpha$.
\end{claim}
\begin{proof}
	\[\Pr[\Fc(T_{y_a})=(q,b_0,b_1)]= \Pr[\Fc(T)=(q,b_0,b_1)|X=a]=\frac{\pr{X=a|\Fc(T)=(q,b_0,b_1)}\cdot\pr{\Fc(T)=(q,b_0,b_1)}}{\pr{X=a}}\]
	Thus we get that
	\[\Pr[\Fc(T_{y_a})=(q,b_0,b_1)]\ge\pr{X=a|\Fc(T)=(q,b_0,b_1)}\cdot\pr{\Fc(T)=(q,b_0,b_1)}\ge\gamma^5\cdot\alpha\]
\end{proof}

%\begin{claim}\label{claim:triplet-resample-SD}
%	Let $Z=(X,Y,T)$ be a triplet (that can be sampled) and let $\Fc$ be a $\full$ $\gamma$-$\forecaster$ for $T$, such that for every $t\in T$, $\Fc(t)=(q,b_0,b_1)$. Let $a,\nu$ be a constants such that $a\in\zo$ and $\size{a-q}<\nu$. Then one of the following must hold
%	\begin{enumerate}
%		\item $(V,T)$ is statistically $(2\nu+100\sqrt{\gamma})$-close to $(U_q,T)$.
%		\item There exists $\Fc'$ a $\full$ $\gamma$-$\forecaster$ (that can be constructed in poly-time, given access to $\Fc$) for $T$ such that $\Price_Z(\Fc)-\Price_Z(\Fc')\geq \gamma$.
%	\end{enumerate}
%	We stress out that the claim holds only when the pair $(X,T)$ can be sampled in poly-time.
%\end{claim}

\begin{lemma}\label{lemma:Full to Partial forecaster distinguishing}
	Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ be a $\gamma$-$\forecaster$. Denote by $\Fc_1,\Fc_2,\Fc_3$ the three $\fpartial$ $\gamma$-$\forecaster$ that compose $\Fc$. Let $q_1,q_2,q_3,\nu,\alpha$ be constants such that $w=(q_1,q_2,q_3)\in\cW_{\gamma}^3$ and define the three pairs: $Z_1=(V_1,T_1)=(X,T)$, $Z_{2}=(V_{2},T_{2})=((Y,T)|X=0)$ and $Z_{3}=(V_{3},T_{3})=((Y,T)|X=1)$. For every index $i\in\{1,2,3\}$, if $\pr{\Fc(T_i)=w}>\alpha>\gamma^7$, $\nu\le q_i \le 1-\nu$ and there exists function $\Dc:\zo\times\zn\to\zo$ such that
	$$\pr{\Dc(V_i,T_i)=1|\Fc(T)=w}-\pr{\Dc(U_{\Fc(T_i)},T_i)=1|\Fc(T)=w}>\rho,$$
	then there exists $\Fc^\ast$ a $\gamma$-$\forecaster$ (that we can construct in poly-time given access to $\Fc$ and $\Dc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)>\gamma\cdot(2\rho-\gamma)\cdot\alpha$
\end{lemma}
\begin{proof}
	The proof is a direct conclusion of Lemma \ref{lemma:Partial forecaster distinguishing}. Let $i\in\{1,2,3\}$ be the index for which the assumptions hold, we define the pair $Z_{i}'=(V_{i}',T_{i}')=((V_{i},T_{i})|\Fc(T)=w)$, note that since $\pr{\Fc(T_i)=w}>\alpha>\gamma^7$ the pair $Z_{i}$ can be sampled in poly-time. Thus we can use Lemma \ref{lemma:Partial forecaster distinguishing} on the pair $Z_{i}'$ with $\Fc_i$ and $\Dc$, and we get that there exists $\Fc'$ a $\fpartial$ $\gamma$-\forecaster such that $\Price_{Z_{i}'}(\Fc_i)-\Price_{Z_{i}'}(\Fc')>\gamma\cdot(2\rho-\gamma)$.
	% We now define $\Fc''$ a $\fpartial$ $\gamma$-$\forecaster$ as follows: for every $t\in T$	
	%\[\Fc''(t)= \left\{ \begin{array}{ll}
	%\ \Fc'(t) & \mbox{if } \Fc(t)=w \\
	%\Fc_{i}(t) & \mbox{otherwise }
	%\end{array} \right. \]
	Note that by assumption we have that $\pr{\Fc(T_{i})=w}\ge \alpha$. Thus we get that $\Price_{Z_i}(\Fc_{i})-\Price_{Z_i}(\Fc'')>\Pr[\Fc(T_{i})=w]\cdot (\Price_{Z_{i}'}(\Fc_i)-\Price_{Z_{i}'}(\Fc'))>\gamma\cdot(2\rho-\gamma)\cdot\alpha$.
	
	
	Thus we can now define the new  $\gamma$-$\forecaster$ $\Fc^\ast$ (not $\fpartial$) by defining the three $\fpartial$ $\gamma$-$\forecaster$  that compose it. For every $j\in\{1,2,3\}$ if $j=i$ then $\Fc^\ast_{j}(t)=\Fc''(t)$, else $\Fc_{j}^\ast(t)=\Fc_{j}(t)$. Thus we get that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)>\gamma\cdot(2\rho -\gamma)\cdot\alpha$, and the lemma holds.
\end{proof}




\begin{claim}\label{claim:3 distinguishers}
	Let $Z=(X,Y,T)$ be a triplet and $q,b\in[0,1]$ be constants. Let $\Dc: \zo\times\zo\times\zn\to\zo$ be a function, if $\pr{\Dc(X,Y,T)=1}-\pr{\Dc(U_{q},U_b,T)=1}>\rho$, then one of the following holds:
	\begin{enumerate}
		\item  $\pr{\Dc(X,U_{b},T)=1}-\pr{\Dc(U_{q},U_{b},T)=1}>\frac{\rho}{3}$.
		\item  $\pr{X=0}\cdot\big(\pr{\Dc(0,Y,T)=1|X=0}-\pr{\Dc(0,U_{b},T)=1|X=0}\big)>\frac{\rho}{3}$.
		\item  $\pr{X=1}\cdot\big(\pr{\Dc(1,Y,T)=1|X=1}-\pr{\Dc(1,U_{b},T)=1|X=1}\big)>\frac{\rho}{3}$.
	\end{enumerate}
\end{claim}
\begin{proof}
	Assume for contradiction that the claim does not hold. Then we get that
	$$
	\pr{\Dc(X,Y,T)=1}-\pr{\Dc(X,U_{b},T)=1}\leq \frac{2\rho}{3}.
	$$
	This is because
	\begin{align*}
	\pr{\Dc(X,Y,T)=1}-&\pr{\Dc(X,U_{b},T)=1}=\\
	&+\pr{X=1}\cdot\big(\pr{\Dc(X,Y,T)=1|X=1}-\pr{\Dc(X,U_{b},T)=1|X=1}\big)\\
	&+\pr{X=0}\cdot\big(\pr{\Dc(X,Y,T)=1|X=0}-\pr{\Dc(X,U_{b},T)=1|X=0}\big)\\		
	\end{align*}
	and from the assumption, both point (2) and point (3) in the claim do not hold, and we get that the sum is less than $\frac{2\rho}{3}$.
	To conclude, note that
	\begin{align*}
	\pr{\Dc(X,Y,T)=1}-\pr{\Dc(U_{q},U_{b},T)=1}=&\pr{\Dc(X,Y,T)=1}-\pr{\Dc(X,U_{b},T)=1}\\
	+&\pr{\Dc(X,U_{b},T)=1}-\pr{\Dc(U_{q},U_{b},T)=1}.	
	\end{align*}
	Thus from the calculations above and by the assumption on the first point in the claim, we get that
	$$
	\pr{\Dc(X,Y,T)=1}-\pr{\Dc(U_{q},U_{b},T)=1}\leq \frac{\rho}{3} +\frac{2\rho}{3}=\rho,
	$$
	and this is a contradiction.
\end{proof}




%	\begin{enumerate}
%		\item  $\pr{\Dc'(V_1,T_1)=1|\Fc(T)=w}-\pr{\Dc'(U_{\Fc_1(T_1)},T_1)=1|\Fc(T)=w}>\frac{\rho}{3}$.
%		\item  $\pr{X=0|\Fc(T)=w}\cdot(\pr{\Dc'(V_2,T_2)=1|\Fc(T)=w}-\pr{\Dc'(U_{\Fc_2(T_2)},T_2)=1|\Fc(T)=w})>\frac{\rho}{3}-(q)|b_0-b_1|$.
%		\item  $\pr{X=1|\Fc(T)=w}\cdot(\pr{\Dc'(V_3,T_3)=1|\Fc(T)=w}-\pr{\Dc'(U_{\Fc_3(T_3)},T_3)=1|\Fc(T)=w})>\frac{\rho}{3}-(1-q)|b_1-b_0|$.
%	\end{enumerate}




\begin{lemma}\label{lemma:atom at the edge}
	Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ be a  $\gamma$-$\forecaster$. Let $q,b_0,b_1,b$ be constants, where $q,b_0,b_1\in \cW_\gamma$, $b=qb_1+(1-q)(b_0)$ and $w=(q,b_0,b_1)$. Let $\Dc:\zo\times\zo\times\zn\to \zo$ be a function. If $\pr{\Fc(T)=w}>\gamma^5$, $q\in([0,\nu]\cup [1-\nu,1])$ and  $\pr{\Dc(X,Y,T)=1|\Fc(T)=w}-\pr{\Dc(U_q,U_b,T)=1|\Fc(T)=w}>\rho$ (for $\rho>10\nu+300\sqrt{\gamma}$),
	then there exists $\Fc^\ast$ a $\gamma$-$\forecaster$ (that can be constructed in poly-time given access to $\Dc$ and $\Fc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)\ge \gamma^6\cdot\nu\cdot (2(\frac{\rho}{3}-\nu)-\gamma)>\gamma^8=\mu$.
\end{lemma}
\begin{proof}
Define the three pairs $Z_x=(V_x,T_x)=(X,T)$, $Z_{y_0}=(V_{y_0},T_{y_0})=((Y,T)|X=0)$ and $Z_{y_1}=(V_{y_1},T_{y_1})=((Y,T)|X=1)$, and let $\Fc_x,\Fc_{y_0},\Fc_{y_1}$ denote three $\fpartial$ $\gamma$-$\forecaster$ that compose $\Fc$. Let $B=\set{\Fc(T)=w}$ be an event, by Claim \ref{claim:3 distinguishers} one of the following must hold
	\begin{enumerate}
		\item  $\pr{\Dc(X,U_{b},T)=1|B}-\pr{\Dc(U_{q},U_{b},T)=1|B}>\frac{\rho}{3}$.
		\item  $\pr{X=0|B}\cdot\big(\pr{\Dc(0,Y,T)=1|B,X=0}-\pr{\Dc(0,U_{b},T)=1|B,X=0}\big)>\frac{\rho}{3}$.
		\item  $\pr{X=1|B}\cdot\big(\pr{\Dc(1,Y,T)=1|B,X=1}-\pr{\Dc(1,U_{b},T)=1|B,X=1}\big)>\frac{\rho}{3}$.
	\end{enumerate}

		 Let $K_0,K_1,K_e,K_m$ be intervals in $[0,1]$, such that $K_0=[0,\nu]$,$K_1=[1-\nu,1]$,$K_e=K_0\cup K_1$ and $K_m=(\nu,1-\nu)$. By the assumption in the claim we have that $q\in K_0\cup K_1$, let $a\in\zo$ be the index such that $q\in K_a$, this satisfies the conditions for Claim \ref{claim:triplet-edeg-resample} on the pair $(V_x,T_x)$. If the first point in Claim \ref{claim:triplet-edeg-resample} hold, then there exists $\Fc^\ast$ a $\gamma$-$\forecaster$ such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)>\Pr[\Fc(T_x)=w]\cdot \gamma=\gamma^6>\mu$, as desired in this lemma. But if the second point in Claim \ref{claim:triplet-edeg-resample} hold, and we get that $((V_x,T_x)|B)$ is statistically $(2\nu+100\sqrt{\gamma})$-close to $((U_q,T_x)|B)$, it follows that point (1) of the lemma: $\pr{\Dc(X,U_{b},T)=1|B}-\pr{\Dc(U_{q},U_{b},T)=1|B}>\frac{\rho}{3}$,  can't hold since $(2\nu+100\sqrt{\gamma})<\frac{\rho}{3}$.
		
		
		Thus we can now assume that point (1) above does not hold and that $((V_x,T_x)|B)$ is statistically $(2\nu+100\sqrt{\gamma})$-close to $((U_q,T_x)|B)$. This means that $\pr{X=a|B}>1-(3\nu+100\sqrt{\gamma})$ since $((U_q,T_x)|B)$ and $((a,T_x)|B)$ are $\nu$-statistically close.
			Let $\hat{a}\in\zo$ be defined such that $a\ne\hat{a}$, this means that  $\pr{X=\hat{a}|B}\le3\nu+100\sqrt{\gamma}$. Recall that one of the remaining possibilities from the  points above is
			$$\pr{X=\hat{a}|B}\cdot\big(\pr{\Dc(\hat{a},Y,T)=1|B,X=\hat{a}}-\pr{\Dc(\hat{a},U_{b},T)=1|B,X=\hat{a}}\big)>\frac{\rho}{3},$$	
		%	$$\pr{X=\hat{a}|B}\cdot(\pr{\Dc'(V_{y_{\hat{a}}},T_{y_{\hat{a}}})=1|B}-\pr{\Dc'(U_{\Fc_{y_{\hat{a}}}(T_{y_{\hat{a}}})},T_{y_{\hat{a}}})=1|B})>\frac{\rho}{3}-(1-q)|b_0-b_1|$$
		%	$$\pr{X=\overline{a}|B}\cdot\big(\pr{\Dc(\overline{a},Y,T)=1|X=\overline{a}}-\pr{\Dc(\overline{a},U_{b},T)=1|X=\overline{a}}\big)>\frac{\rho}{3}$$
			but this of course does not hold since $\pr{X=\hat{a}}\le3\nu+100\sqrt{\gamma}$ and $3\nu+100\sqrt{\gamma}<\frac{\rho}{3}$. Thus we are left with one possibility that must hold, and we get that
			$$\pr{X=a|B}\cdot\big(\pr{\Dc(a,Y,T)=1|B,X=a}-\pr{\Dc(a,U_{b},T)=1|B,X=a}\big)>\frac{\rho}{3}.$$  We now define $\Dc':\zo\times\zn\to\zo$ as follows: for every $t\in \zn$ and $v\in\zo$, $\Dc'(v,t)=\Dc(a,v,t)$. and we get that $\pr{\Dc'(V_{y_a},T_{y_a})=1|B}-\pr{\Dc'(U_{b},T_{y_a})=1|B}>\frac{\rho}{3}$. By the following fact,
			\begin{fact}
			For every $a'\in\zo$ such that $q\in K_{a'}$ we have that $|b-b_{a'}|\le \nu$.
			\end{fact}
			\begin{proof}
				By definition we have that $b=qb_1+(1-q)b_0$, thus if $q\in K_1$ this means that $|b-b_1|=|qb_1+(1-q)b_0-b_1|=|(1-q)(b_0-b_1)|\le(1-q)\le\nu.$ And if $q\in K_0$ then we get $|b-b_0|=|qb_1+(1-q)b_0-b_0|=|q(b_1-b_0)|\le q \le \nu.$
			\end{proof}
			It is easy to see that $((U_{b},T_{y_a})|B)$ and $((U_{b_a},T_{y_a})|B)$ are statistically $\nu$-close as follows from the above claim. Thus we get that
			$$\pr{\Dc'(V_{y_a},T_{y_a})=1|B}-\pr{\Dc'(U_{b_a},T_{y_a})=1|B}>\frac{\rho}{3}-\nu.$$
		%	Recall that by definition $\pr{\Fc_{y_{a}}(T)=b_a|B}=1$ $\Fc$
			First note that since $\pr{X=a|B}>1-(3\nu+100\sqrt{\gamma})$ by Claim \ref{claim:conditional atoms size} we have that $\pr{\Fc(T_{y_a})=w}\ge \gamma^5\cdot\nu$.
		    There are two remaining cases to consider depending on the value of $b_a$, both of which give us $\Fc^\ast$ a $\gamma$-$\forecaster$ such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)>\Pr[\Fc(T_{y_a})=w]\cdot \gamma(2(\frac{\rho}{3}-\nu)-\gamma)=\nu\cdot\gamma^6\cdot (2(\frac{\rho}{3}-\nu)-\gamma)>\gamma^8=\mu$ as desired in the lemma.
			
			 If $b_a\in K_m$, we use Lemma \ref{lemma:Full to Partial forecaster distinguishing} that gives us $\Fc^\ast$ as stated. But if $b_a\in K_e$ then in this case we initiate Claim \ref{claim:triplet-edeg-resample} again this time on the pair $(V_{y_a},T_{y_a})$, recall that $\pr{\Dc'(V_{y_a},T_{y_a})=1|B}-\pr{\Dc'(U_{b_a},T_{y_a})=1|B}>\frac{\rho}{3}-\nu$ thus $((V_{y_a},T_{y_a})|B)$ can't be statistically $(2\nu+100\sqrt{\gamma})$-close to $((U_{b_a},T_{b_a})|B)$, since $(2\nu+100\sqrt{\gamma}) <\frac{\rho}{3}-\nu$. Consequently the second point in Claim \ref{claim:triplet-edeg-resample} can't hold and we are left with the first point that guarantees $\Fc^\ast$ as desired.
\end{proof}	


\begin{lemma}\label{lemma:atom in the middle}
	Let $Z=(X,Y,T)$ be a triplet and let $\Fc$ be a $\gamma$-$\forecaster$. Let $q,b_0,b_1,b$ be constants, where $q,b_0,b_1\in \cW_\gamma$, $b=qb_1+(1-q)(b_0)$ and $w=(q,b_0,b_1)$. Let $\Dc:\zo\times\zo\times\zn\to \zo$ be a function. If $\pr{\Fc(T)=w}>\gamma^5$, $\nu<q<1-\nu$, $\size{b_0-b_1}<\lambda$ and  $\pr{\Dc(X,Y,T)=1|\Fc(T)=w}-\pr{\Dc(U_q,U_b,T)=1|\Fc(T)=w}>\rho$,
 then there exists $\Fc'$ a $\gamma$-$\forecaster$ (that can be constructed in poly-time given access to $\Dc$ and $\Fc$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc')>\gamma^6\cdot(\nu-100\sqrt{\gamma})\cdot(2(\frac{\rho}{3}-\lambda)-\gamma)\ge\mu$, for $\mu=\gamma^8$.
\end{lemma}
\begin{proof}
	Define the three pairs $Z_1=(V_1,T_1)=(X,T)$, $Z_{2}=(V_{2},T_{2})=((Y,T)|X=0)$ and $Z_{3}=(V_{3},T_{3})=((Y,T)|X=1)$. Let $B=\set{\Fc(T)=w}$ be an event and let $\Fc_1,\Fc_2,\Fc_3$ denote the three $\fpartial$ $\gamma$-$\forecaster$ for $\Fc$. By Claim \ref{claim:3 distinguishers} on of the following must hold
	\begin{enumerate}
		\item  $\pr{\Dc(X,U_{b},T)=1|B}-\pr{\Dc(U_{q},U_{b},T)=1|B}>\frac{\rho}{3}$.
		\item  $\pr{X=0|B}\cdot\big(\pr{\Dc(0,Y,T)=1|B,X=0}-\pr{\Dc(0,U_{b},T)=1|B,X=0}\big)>\frac{\rho}{3}$.
		\item  $\pr{X=1|B}\cdot\big(\pr{\Dc(1,Y,T)=1|B,X=1}-\pr{\Dc(1,U_{b},T)=1|B,X=1}\big)>\frac{\rho}{3}$.
	\end{enumerate}
			First note since $\pr{\Fc(T)=w}\ge\gamma^5$, we can initiate Claim \ref{claim:dist from exp imply better partial forecaster} for the pair $(X,T)$. If the first point in Claim \ref{claim:dist from exp imply better partial forecaster} hold, then we get $\Fc'$ a $\gamma$-$\forecaster$ such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc')>\gamma\cdot\pr{\Fc(T)=w}\ge\gamma^6$ as desired in the lemma and the proof is complete. Thus we can now assume that the second point in Claim \ref{claim:dist from exp imply better partial forecaster} holds, and we get that
			$$\nu-100\sqrt{\gamma}<\pr{X=1|B}<1-\nu+100\sqrt{\gamma}.$$
			Note that this implies that for every $i\in\{1,2,3\}$, $\Pr[\Fc(T_i)=w]\ge(\nu-100\sqrt{\gamma})\cdot\pr{\Fc(T)=w}\ge (\nu-100\sqrt{\gamma})\cdot\gamma^5$ as follows from Claim \ref{claim:conditional atoms size}.
	
	\begin{claim}
		There exists $\Dc':\zo\times\zn\to\zo$ (which can be constructed in $\poly$-time given access to $\Dc$) and $i\in\{1,2,3\}$ such that: $\pr{\Dc'(V_i,T_i)=1|B}-\pr{\Dc'(U_{\Fc_i(T_i)},T_i)=1|B}>\frac{\rho}{3}-\lambda$.
	\end{claim}	
	\begin{proof}
			 By Claim \ref{claim:3 distinguishers}, at least on of the above points must hold. If point (1) holds, then by averaging there exists a fixed $a\in\zo$ such that
			 $
			 \pr{\D(X,a,T)=1|B}-\pr{\D(U_q,a,T)=1|B}>\frac{\rho}{3}
			 $
			 (we can find this fixed "a" be sampling and trying both possible values), and so we can make the following definition: for every $v\in \zo$ and $t \in \zn$, $\Dc'(v,t)=\Dc(v,a,t)$, and the claim follows.
			 % And since $\pr{\Fc_1(T_1)=q|B}=1$, we get $\pr{\Dc'(V_1,T_1)=1|B}-\pr{\Dc'(U_{\Fc_1(T_1)},T_1)|B}>\frac{\rho}{3}$.
			
			  But if point (2) or (3) hold, then we do things a little differently. We define $\Dc_2,\Dc_3:\zo\times\zn\to \zo$ as follows, for every $v\in\zo$ and $t \in \zn$: $\Dc_2(v,t)=\Dc(0,v,t)$ and $\Dc_3(v,t)=\Dc(1,v,t)$. We get that there exists $j\in\{2,3\}$ such that:
			 \begin{equation}\label{eq: dist 1}
			 \pr{\Dc_j(V_j,T_j)=1|B}-\pr{\Dc_j(U_{b},T_j)=1|B}>\frac{\rho}{3}.
			 \end{equation}
			 \begin{fact}\label{fact:SD for bits}
			 	Let $q_1,q_2\in[0,1]$ and $\lambda'$ be constant such that $|q_1-q_2|<\lambda'$ then $\SD(U_{q_1},U_{q_2})<\lambda'$.
			 \end{fact}
			 By the above, for every $i\in\{0,1\}$ have that $((U_{b_i},T)|B)$ and $((U_{b},T)|B)$ are $\lambda$-statistically close, since by the assumption $|b_1-b_0|<\lambda$ and as such $|b_i-b|<\lambda$.
			 Recall that by definition $\pr{\Fc_2(T_2)=b_0|B=1}=1$ and $\pr{\Fc_3(T_3)=b_1|B=1}=1$, thus we get that for every $j\in \{2,3\}$
			 \begin{equation} \label{eq: dist 2}
			 \pr{\D_j(U_{b},T_j)=1|B} -\pr{\D_j(U_{\Fc_j(T_j)},T_j)=1|B}> -\lambda.
			 \end{equation}
			 Combining the above two equations, we get	
			 \begin{equation}
			 \pr{\Dc_j(V_j,T_j)=1|B}-\pr{\D_j(U_{\Fc_j(T_j)},T_j)=1|B}= (\ref{eq: dist 1})+(\ref{eq: dist 2})>\frac{\rho}{3}-\lambda,
			 \end{equation}
			 and since Claim \ref{claim:3 distinguishers} guarantees that on of the points hold, this concludes the proof.
	\end{proof}
		
	\begin{claim}\label{claim:distinguishing for partial to full}
	Given $i\in \{1,2,3\}$ and a function $\Dc':\zo\times\zn\to\zo$ such that
	$\pr{\Dc'(V_i,T_i)=1|B}-\pr{\Dc'(U_{\Fc_i(T_i)},T_i)=1|B}>\frac{\rho}{3}-\lambda$,
	there exists $\Fc^\ast$ a $\gamma$-$\forecaster$ (that can be constructed in poly-time given access to $\Dc'$) such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)\ge  \gamma^5\cdot(\nu-100\sqrt{\gamma})\cdot\gamma\cdot(2(\frac{\rho}{3}-\lambda)-\gamma)\ge\mu$, for $\mu=\gamma^8$.
\end{claim}
\begin{proof}
	Let $i\in \{1,2,3\}$ be the index referred to in the claim. If $\pr{\nu <\Fc_i(t)<1-\nu|B}=1$ we use Lemma \ref{lemma:Full to Partial forecaster distinguishing}
	%(the lemma and proof are in the second subsection that deals with the $\fpartial$ \forecaster )
	that gives us $\Fc^\ast$ as stated in the claim. Otherwise $\pr{\Fc_i(t)\in ([0,\nu]\cup [1-\nu,1])|B}=1$ and in this case we initiate Claim \ref{claim:triplet-edeg-resample} on the pair $(V_i,T_i)$, recall that $\pr{\Dc'(V_i,T_i)=1|B}-\pr{\Dc'(U_{\Fc_i(T_i)},T_i)=1|B}>\frac{\rho}{3}-\lambda$ thus $((V_i,T_i)|B)$ can't be statistically $(2\nu+100\sqrt{\gamma})$-close to $((U_{\Fc_i(T_i)},T_i)|B)$, since $(2\nu+100\sqrt{\gamma}) <\frac{\rho}{3}-\gamma$. Consequently the second point in Claim \ref{claim:triplet-edeg-resample} can't hold and we are left with the first point that guarantees $\Fc^\ast$ as desired.
\end{proof}
The proof follows by the above two claims.
\end{proof}

We are now ready to prove Lemma \ref{lemma:Distinguishing to better forecasting} which will make use of the above claims can lemmas in this section.

\begin{proof}(proof of Lemma \ref{lemma:Distinguishing to better forecasting})
	We define the function $C:\cW_\gamma^3\to [0,1]$ such that for every $q,b_0,b_1\in\cW_\gamma$, $C(q,b_0,b_1)=\pr{\Fc(T)=(q,b_0,b_1)}$\jnote{(we should argue that we have $C'$ a function that samples and is close to function $C$ with high probability)}. Let $H\subseteq \cW_\gamma^3$ be a set defined as follows, $H=\set{(q,b_0,b_1)\colon q,b_0,b_1\in\cW_\gamma, C(q,b_0,b_1)>\gamma^5}$, note that $\pr{\Fc(T)\notin H}\leq\size{\cW_\gamma^3}\cdot\gamma^5=\gamma^2$. Let $G=G_0\cup G_1\cup G_2$ denote an event, we get that
	\[ \pr{\Dc(X,Y,T)=1|G,\Fc(T)\in H}-\pr{\Dc(U_{\Fc_x(T)},U_{\Fc_y(T)},T)=1|G,\Fc(T)\in H} >\rho-\gamma^2-\beta=\rho'\]
	This means that there exists a fixed $w=(q,b_0,b_1)\in H$ such that $q\in([0,\nu]\cup[1-\nu,1])$ or $|b_0-b_1|<\lambda$ (which we can sample and find)\jnote{(which we can sample and find, we need to deal with the sampling error)} and it holds that
	\[ \pr{\Dc(X,Y,T)=1|\Fc(T)=w}-\pr{\Dc(U_{q},U_{b},T)=1|\Fc(T)=w} >\rho'\]
	We now have two possibilities that depend on $w=(q,b_0,b_1)$ that we chose. If $q\in([0,\nu]\cup[1-\nu,1])$ then we initiate Lemma \ref{lemma:atom at the edge}, otherwise we have that $\nu<q<1-\nu$ and $|b_0-b_1|<\lambda$ and we can initiate Lemma \ref{lemma:atom in the middle}, in both cases we can construct a $\gamma$-$\forecaster$ $\Fc^\ast$ such that $\Price_{Z}(\Fc)-\Price_{Z}(\Fc^\ast)>\mu$ for $\mu=\gamma^8$, and the lemma holds.
\end{proof}


%\jnote{We use a reduction to the partial forecaster setup, we prove the existence of a distinguisher for one of the partial forecasters but to know which one it is we need to sample the three distributions. I am not sure if this can work, since we can fail with some probability. And this further shows that we have to deal with probabilistic forecasters.}


%\jnote{here I am assuming that after the conditioning the pairs $Z_2,Z_3$ are well defined}






==> MainThm.tex <==


\section{Proving  The Dichotomy of Two-Party Protocols}\label{sec:proofMainThm}
In this section we the main result of \cref{sec:Forecasters,sec:ForecastingToKA} to prove our main theorem.
\begin{theorem}[Main theorem, restated]\label{thm:mainRes}
	\MainThm
\end{theorem}
\begin{proof}
Let  $\rho>0$, let $\pi$ be a \ppt single-bit output two-party protocol, and let  $Z_\kappa= (X_\kappa,Y_\kappa,T_\kappa)$ be the distribution of the parties' output and protocol transcripts induce by a random execution of $\pi(1^\kappa)$.  Let $\rho' = (60\rho)^2$. By \cref{thm:one:Indist} exists a  forecaster \Fc	that is $(\rho',\I')$-indistinguishable \wrt $Z= \set{x_\kappa}$, for an infinite set $\I' \subseteq \I$. If there exists an infinite subset $\I'' \subseteq \I'$ for which $\Fc$  is $(\rho/2,\I'')$-correlated \wrt $Z$, then by \cref{cor:full KA from correlation}, there exists a two-party io key-agreement protocol. 

Otherwise, let $\Decr(1^\kappa,t;r) = \Prod(\Fc(1^\kappa,t;r))$ for $\Prod(p)$ be the product distribution defined by the  marginal of the distribution defined by $p$ (see \cref{nota:ProdOfDis}).  \cref{prop:UncorrelationPlusIndistToProd} yields that $\Decr$ is a $(\rho'+ \rho/2 < \rho,\I')$-decorelator for $\pi$.    
\end{proof}

==> TheAttack.tex <==
\section{Definitions for DP and $\mech$.}\label{sec:Attack}

In this section we will recall the basic notion of differential privacy, and then define $\mech$, which can be derived from a standard definition of DP.  

\begin{definition}[Computational differential privacy,\cite{MPRV09}]
	\label{def:IND-CDP}
	An ensemble $\{f_\pk\}_{\pk\in\N}$ of randomized functions $f_\pk:\mathcal{D}\rightarrow \mathcal{R}_\pk$ provides {\sf$\eps_\pk$-\INDCDP} if there exists a negligible function $\negl(.)$ such that for every nonuniform \pptm ("distinguisher") $\Ac$, every polynomial $p\in \poly$, every sufficiently large $\pk\in\N$, all data sets $\cD,\cD'\in\mathcal{D}$ of size at most $p(\pk)$  such that $|\cD\Delta \cD'|\leq 1$, and every advice string $z_\pk$ of size at most $p(\pk)$, it holds that
	\[\Pr[A_\pk(f_\pk(D))=1]\leq e^{\eps_{\pk}}\times \Pr[A_\pk(f_\pk(D'))=1]+\negl(\pk),\]
	where we write $A_\pk(x)$ for $A(1^\pk,z_\pk,x)$ and the probability is taken over the randomness of mechanism $f_\pk$ and adversary $A_\pk$.
\end{definition}




\begin{definition}[Differentially private XOR]
	\label{def:DP-XOR}
	We say that an ensemble $\{M_\pk\}_{\pk\in\N}$ of randomized functions $M_\pk:\zo\times\zo\rightarrow \mathcal{R}_\pk$ is  {\sf$\eps_\pk$-\INDCDP} and $\delta$-accuracy with respect to the XOR function. If there exists a negligible function $\negl(.)$ such that for every nonuniform \pptm ("distinguisher") $\Ac$, every polynomial $p\in \poly$, every sufficiently large $\pk\in\N$, all pairs of $(x,y),(x',y')\in\zo\times\zo$  such that $|(x,y)\Delta (x',y')|\leq 1$, and every advice string $z_\pk$ of size at most $p(\pk)$, it holds that
	
		\begin{enumerate}
			\item Security:
					\[\pr{A_\pk(M_\pk((x,y)))=1}\leq e^{\eps_{\pk}}\times \pr{A_\pk(M_\pk((x',y')))=1}+\negl(\pk).\]
			\item Accuracy:
	
		\[\pr{x\xor y=Output(M_\pk(x,y))}\ge\half+\delta.\] 

		\end{enumerate}
	
	where we wright $A_\pk(x)$ for $A(1^\pk,z_\pk,x)$ and the probability is taken over the randomness of mechanism $M_\pk$ and adversary $A_\pk$.
	
\end{definition}

\jnote{We probably need the (Two-Party protocol for differentially private XOR) and not the above definition.}
\begin{definition}[Two-Party protocol for differentially private XOR.]
	\label{def:DP-XOR-Protocol}
	Let $\set{\prot_\secParam\eqdef(\Ac,\Bc)(1^\secParam)}_{\secParam\in\N}$ be an ensemble of interactive protocol where the inputs of $\Ac$ and $\Bc$ are in $\zo$. We say that $\set{\prot_\secParam}_{\secParam\in\N}$ is an {\sf $(\eps_\secParam,\delta_\secParam)$-$\XOR$ protocol} if
	\begin{enumerate}
		\item For every $x\in\zo$ the ensemble $\set{\view^{\Ac}_{\pi}(\secParam,x,\cdot)}_{\secParam\in\N}$ provides $\eps_\secParam$-\INDCDP over inputs of $y\in\zo$.
		\item For every $y\in\zo$ the ensemble $\set{\view^{\Bc}_{\pi}(\secParam,\cdot,y)}_{\secParam\in\N}$ provides $\eps_\secParam$-\INDCDP over inputs of $x\in\zo$.
		\item For every $x,y\in\zo$, $\pr{\out_\pi(x,y)=x\xor y}\ge\half+\delta_\secParam$.
	\end{enumerate}
	
\end{definition}








\section{The construction}\label{sec:construction}

\subsection{DP Triplet}


\begin{definition}[Differentially private triplet]\label{def:DP-Triplet-Var}
For every $\secParam\in\N$ we say that the random variable $Z_\secParam=(\XYTp)$ over $\zo\times\zo\times\zo^\pk]$ is an {\sf $(\eps_\secParam,\delta_\secParam)$-\dpt}, if there exists a negligible function $\negl(.)$ such that for every nonuniform \pptm ("distinguisher") $\Fc$, every polynomial $p\in \poly$, and every advice string $z_\secParam)$ of size at most $p(\secParam))$, it holds that
\item Security: if $\pr{\Fc_\secParam(T_\secParam)=1}> noticeable(\secParam)$ \Inote{??} then 
\begin{itemize}
	\item $\pr{X_\secParam=1|Y_\secParam=y',\Fc_\secParam(T_\secParam)=1}\in [\half - \eps_\secParam,\half+\eps_\pk]$ for  every $y'\in\zo$.	
	\item $\pr{Y_\pk=1|X_\pk=x',\Fc_\pk(T_\pk)=1}\in [\half - \eps_\pk,\half+\eps_\pk]$ for  every $x'\in\zo$.
\end{itemize}
\item Accuracy:
\begin{itemize}
	\item $\Pr[X_\pk=Y_\pk]\ge\half+\delta_\pk$.
\end{itemize}
Where we wright $\Fc_\pk(x)$ for $\Fc(1^\pk,z_\pk,x)$ and the probability is taken over $Z_\pk$ the randomness of $\Fc_\pk$.
	

\end{definition}

\begin{definition}[Ensemble of differentially private triplets]\label{def:Ensemble-DP-Triplet}
	
	An ensemble $Z=\set{Z_\pk}_{\pk\in\N}$ of random variables $Z_\pk=(\XYTp)$ over $\zo\times\zo\times\zo^\pk$ is an {\sf $(\eps_\pk,\delta_\pk)$-\EnDpt}, if for every sufficiently large $\pk\in\N$, the random variable $Z_\pk$ is an  $(\eps_\pk,\delta_\pk)$-\dpt. 

\end{definition}


\begin{definition}[Two-Party protocol for a private DP triplet]
	Let $\set{\prot_\pk\eqdef(\Ac,\Bc)(1^\pk)}_{\pk\in\N}$ be an ensemble of interactive protocol where the inputs of $\Ac$ and $\Bc$ are in $\zo$. We say that $\set{\prot_\pk}_{\pk\in\N}$ is an {\sf $(\eps_\pk,\delta_\pk)$-\dpt protocol} if for every sufficiently large $\pk\in\N$, the random variables $X_\pk$ and $Y_\pk$ are the private outputs of $\Ac$ and $\Bc$ respectively, $T_\pk$ is the transcript of the protocol, such that $Z_\pk=(\XYTp)$ is an $(\eps_\pk,\delta_\pk)$-\dpt.    
\end{definition}


\jnote{This is very suspicious, as it seems to me that we are asking very little compared to what we can ask in DP protocol. In the usual DP protocol the security is for the view of both players, but here we ask for something weaker.}



\begin{figure}[h!]
	\begin{small}
		\begin{center}
			\caption{\dpt protocol: The two parties $(\Ac,\Bc)$ generates a \dpt random variable from a $\XOR$ protocol.}
			\label{fig:Triplet-Protocol}
		\begin{tabular}{|p{16cm}|c|}
			\hline
			\begin{description}
				\item[Parameters: ] $\mbox{}$
				\begin{itemize}	
					\item $\secParam$ - A security parameter that is given as an input.
					\item $\eps$ - The privacy parameter for a $\XOR$ protocol.
					\item $\delta$ - The accuracy parameter for a $\XOR$ protocol.
				\end{itemize}				
	%			\item[Internal parameters: ] $\mbox{}$
	%			\begin{itemize}	
	%				\item $\gamma$ - Will be chosen as a function of $\delta$ and determines the range of the \forecaster. This is a constant.
					%	\item $\mu$ -The minimality parameter of an \forecaster. $\mu$ is a constant that depends on $\delta$ and will be chosen later.   
	%			\end{itemize}
				\item[Ingredients: ] $\mbox{}$
				\begin{itemize}
					%\item  $\prot_\secParam$ - An $(\eps,\delta)$-$\XOR$ protocol. 
					\item  $\set{\prot_\secParam}_{\secParam\in\N}$ - An ensemble of $(\eps,\delta)$-$\XOR$ protocol.
					%\item  $\prot_\secParam	\eqdef(\Ac',\Bc')(1^\secParam)$ - An $(\eps,\delta)$-$\XOR$ protocol.
					%	\item $\edp=\enXYTp$ - An ensemble of random variables that is  $(\eps,\delta)$-$\dpt$. 
				\end{itemize}
				
				\item[Operation of the \dpt protocol $(\Ac,\Bc)$: ] $\mbox{}$
			%	\begin{description}
			%	\end{description}
				\begin{description}
					\item[Common inputs:] security parameter $1^\secParam$ .
					
					\item[$\Ac$'s inputs:] $x \in \zo$. 

					\item[$\Bc$'s inputs:] $y \in \zo$.
					
					 \item[Operation: ] $\mbox{}$
						\begin{enumerate}							
							\item Parties $\Ac$ and $\Bc$ invoke the $\XOR$ protocol $\pi_\secParam$ with input $(x,y)$, and both receive $z=\out_{\pi_{\secParam}}(x,y)$. 
							\item If $z=0$ then the parties $\Ac$ and $\Bc$ set their privet output to $x$ and $y$ respectively.
							\item Otherwise $z=1$, both parties output an independent  uniform  bit. \jnote{Not sure about this..}  	
						\end{enumerate}
				\end{description}
			\end{description}
			
			\\ \hline
		\end{tabular}
	\end{center}
\end{small}
\end{figure}

\subsection{Definition for the forecaster and the Price function}

\begin{definition}[$\cW_\gamma$]\label{def:W-Set}
	For constant $\frac{1}{4}>\gamma>0$, we define the  finite set
	$$
	 \cW_\gamma=\set{\half+i\gamma \colon i\in\Z, -\frac{1}{4\gamma}<i<\frac{1}{4\gamma}}.
	 $$
\end{definition}
We refer to $\cW_\gamma$ as the range of $\gamma$, and we will omit the subscript $\gamma$ when it is clear from the context.  

\begin{definition}[\forecaster]\label{Def:forecaster}
	
	Let $\edp=\enXYTp$ be an $(\eps_\pk,\delta_\pk)$-$\EnDpt$ and let $\gamma> 0$ to be a constant. For an algorithm $\Fc$, we make the following definitions:
	\begin{itemize}
		
		\item $\Fc$ is a {\sf $\singular$ $\gamma$-$\forecaster$} for $\edp$, if for every $\pk\in\N$ it holds that for every $t\in\Supp(T_\pk)$, $\Fc_\pk(t)\in \cW_\gamma$.
		
		\item  $\Fc$ is a {\sf $\gamma$-$\forecaster$} for $\edp$, if for every $\pk\in\N$ it holds that for every $t_1,t_2\in\Supp(T_\pk)$, $\Fc_\pk(t_1,t_2)\in \cW_\gamma\times \cW_\gamma$.
		
		\item $\Fc$ is an {\sf$\oblivious$ $\gamma$-$\forecaster$} for $\edp$, if there exists a $\singular$ $\gamma$-$\forecaster$ $\Fc'$ such that for every $\pk\in\N$ it holds that for every $t_1,t_2\in\Supp(T_\pk)$, $\Fc_\pk(t_1,t_2)=(\Fc'_{\pk}(t_1),\Fc'_{\pk}(t_2))$.   

	\end{itemize}
Where we write $\Fc_\pk(t_1,t_2)$ for $\Fc(t_1,t_2,1^n)$ and $\Fc'_\pk(t)$ for $\Fc'(t,1^n)$, and we will omit the subscript $n$ when it is clear from the context. 
\end{definition}


\begin{definition}[cost function]\label{Def:CostFunction}
	For every  $x\in\zo$ and $p\in[0,1]$, we define 
	$$
	\cost(x,p)=(x-p)^2.
	$$
\end{definition}


\begin{definition}[price function]\label{Def:PriceFunction}
	Given a $\gamma$-$\forecaster$ $\Fc$ for $\EnDpt$ $\edp=\enXYTp$, for every $\pk\in\N$, $x_1,x_2\in\zo$ and $t_1,t_2\in\Supp(T_\pk)$, we define 
	$$
	\price_{\Fc_\pk}(x_1,x_2,t_1,t_2)=\cost(x_1,\Fc_\pk(t_1,t_2)_1)+\cost(x_2,\Fc_\pk(t_1,t_2)_2).
	$$
\end{definition}


\begin{definition}[price for a $\forecaster$]\label{def:Price-Eval}
	Given a $\gamma$-$\forecaster$ $\Fc$ for $\EnDpt$ $\edp=\enXYTp$. Let the $Z^1=\enXYTpo$ and $Z^2=\enXYTpt$ denote two independent copies of $\edp$, 
	\begin{enumerate}
		\item the {\sf value of $\Fc$} is defined as $V(\Fc)=\set{V(\Fc_\pk)}_{\pk\in\N}$ where for every $\pk\in\N$ 
		\[V(\Fc_\pk)=\Ex[\price_{\Fc_\pk}(X^1_\pk,X^2_\pk,T^1_\pk,T^2_\pk)].\]
		
		\item For a series of random event $B=\set{B_\pk}_{\pk\in\N}$, we define the {\sf conditional value of $\Fc$} as $V(\Fc|B)=\set{V(\Fc_\pk|B_\pk)}_{\pk\in\N}$ where for every $\pk\in\N$
		\[V(\Fc_\pk|B_\pk)=\Ex[\price_{\Fc_\pk}(X^1_\pk,X^2_\pk,T^1_\pk,T^2_\pk)|B_\pk].\]   
	\end{enumerate} 

\end{definition}
Namely, $V(\Fc_\pk)$ is the value that measures how far $\Fc_\pk$ is from being "truthful". 	



\section{The KA Protocol.}


\begin{figure}[h!]
	\begin{small}
		\begin{center}
			\caption{KA Protocol: two parties A and B want to agree on secret key}
			\label{fig:KA-Protocol}
			\begin{tabular}{|p{16cm}|c|}
				\hline
				\begin{description}
					\item[Parameters: ] $\mbox{}$
						\begin{itemize}	
						\item $\secParam$ - A security parameter that is given as an input.
						\item $\eps$ - The privacy parameter for a \dpt protocol. This is a constant (for now).
						\item $\delta$ - The accuracy parameter for a \dpt protocol. This is a constant (for now).
						\item $0<p^\ast<1$ - A parameter that is given. $p^\ast$ is a constant that is chosen form a finite set, the possible values that can be assigned to $p^\ast$ depend on $\delta$.
						\end{itemize}				
					\item[Internal parameters: ] $\mbox{}$
					\begin{itemize}	
						\item $\gamma$ - Will be chosen as a function of $\delta$ and determines the range of the \forecaster. This is a constant.
					%	\item $\mu$ -The minimality parameter of an \forecaster. $\mu$ is a constant that depends on $\delta$ and will be chosen later.   
					\end{itemize}
					\item[Ingredients: ] $\mbox{}$
					\begin{itemize}
						\item  $\set{\DPpi_\pk}_{\pk\in\N}$ - An $(\eps,\delta)$-$\dpt$ protocol such that, for security parameter $\pk$ and uniform random input, $\edp_\pk=(\XYTp)$ is the random variable that denotes the output of $\DPpi_\pk$.    	
					%	\item $\edp=\enXYTp$ - An ensemble of random variables that is  $(\eps,\delta)$-$\dpt$. 
						\item $\Fc$ - An algorithm that is a $\gamma$-\forecaster.   
					\end{itemize}
	
					\item[Operation of the protocol, KA $(\Ac,\Bc)$: ] $\mbox{}$
					\begin{description}
						\item[Common inputs:] security parameter $1^\pk$.
									
			%			\item[$\Ac$'s inputs:] $r_\Ac^1,r_\Ac^2\in\zo$, two "radnom" bits. 
	
			%			\item[$\Bc$'s inputs:] $r_\Bc^1,r_\Bc^2\in\zo$, two "radnom" bits.
						
						\item [Operation: ]$\mbox{}$
						
							\begin{enumerate}
								
								\item The parties $\Ac$ and $\Bc$ invoke the protocol $\DPpi_\pk$ twice with independent randomness. Such that $z^1_\pk=(x^1_\pk,y^1_\pk,t^1_\pk)$ and $z^2=(x^2_\pk,y^2_\pk,t^2_\pk)$ denote the first and second output.
								\begin{itemize}
										\item Party $\Ac$ receives the private output $x^1_\pk$ and $x^2_\pk$.
										\item Party $\Bc$ receives the private output $y^1_\pk$ and $y^2_\pk$.
										\item $t^1_\pk$ and $t^2_\pk$ are the transcript for the protocol that are visible to all observers.
								\end{itemize}
						
								\item Party $\Ac$ computes $(p_1,p_2) \la \Fc_\pk(t^1_\pk,t^2_\pk)$.
								
								\item 	If  $p_1=p_2=p^\ast$ and $x^1_\pk\ne x^2_\pk$, it sends $"\YES"$ to $\Bc$, and outputs $x^1_\pk$. $\Bc$ outputs $y^1_\pk$.
								
								Otherwise, $\Ac$ sends  $"\NO"$ to $\Bc$, and both parties output an independent  uniform  bit.
								
							\end{enumerate}

					\end{description}
				\end{description}
				
				\\ \hline
			\end{tabular}
		\end{center}
	\end{small}
\end{figure}





%\section{$\mech$ Implies KA Protocol.}

%\subsection{The KA Protocol and the Attach Eve.}

%\begin{protocol}[Key agreement protocol $(\Ac,\Bc)$ from a XOR DP triplet]
	
%	\item[Parameter:] $\gamma$ and $p^\ast\in \cW_\gamma$. \Inote{$p^\ast$}
	
	 
%	\item[Common inputs:] $t_1,t_2 \in \Supp(T)$. 
	
%	 \item[Oracle:] $\gamma$-\forecaster $\Fc$ for a XOR triplet $Z=(X,Y,T)$.
	 
%	 \item[$\Ac$'s inputs:] $x_1,x_2 \in \Supp(X)$. 
	 
%	 \item[$\Bc$'s inputs:] $y_1,y_2 \in \Supp(Y)$. 
	 
%	 \item Operation:
	 

	
%	\begin{enumerate}
		
%		\item $\Ac$ computes $(p_1,p_2) = \Fc(t_1,t_2)$.
	
	
%		\item 	If  $p_1=p_2=p^\ast$ and $x_1\ne x_2$, it sends $1$ to $\Bc$, and outputs $x_1$. $\Bc$ outputs $y_1$.
		
%		Otherwise, $\Ac$ sends  $0$ to $\Bc$, and both parties output an independent  uniform  bit.
		
%	\end{enumerate}
		
%\end{protocol}
%\Inote{See above changes. Cleanest way is that if parties get wrong inputs, then they output a uniform bit}

%\jnote{Not sure how to change Algorithm to Protocol}

%\begin{theorem}
%	This should be a theorem that states everything together.... later.
%\end{theorem}


\section{Correctness of the KA Protocol}




\begin{theorem}
	Let $\eps,\delta$ be constants as 
\end{theorem}
	






\subsection{The Definition and Existence of a Minimal Forecaster.}

\begin{definition}[minimal \forecaster] 
	Let $\eps,\delta,\gamma,\mu>0$ be constants, and let $K\subset TM$ be the family of every $\gamma$-$\forecaster$ for a $(\eps,\delta)$-$\EnDpt$ $\edp$.
	We say that $\Fc\in K$ is an {\sf $(\mu,\gamma)$-$\minimal$ $\forecaster$} for $\edp$, if there
	exists an {\sf $\infinite$} subset $\I\subseteq\mathbb{N}$, so that
	for every $\Fc'\in K$, exists a {\sf $\finite$} subset $\cS\subseteq\mathbb{N}$, such that for every $n\in (\I \setminus \cS),  V(\Fc_{\pk}')\ge V(\Fc_\pk)-\mu$.
\end{definition}




\begin{lemma}[minimal \forecaster]
	\label{lemma:minimal-forecaster}
		Let $\eps,\delta,\gamma,\mu>0$ be constants. For every $(\eps,\delta)$-$\EnDpt$ $\edp$,  there exists an $(\mu,\gamma)$-$\minimal$ $\forecaster$ $\Fc$ for $\edp$.  
\end{lemma}

\begin{proof}
	The proof idea is direct, will start with an arbitrary $\gamma$-$\forecaster$ each time iteratively replacing it with a "better" $\forecaster$ until a $\minimal$ $\forecaster$ is found. 
	
	
	Let $K\subset TM$, and $\I,\I',\cS\subseteq\N$, we define $K$ to be the family of every $\gamma$-$\forecaster$ for $\EnDpt$ $\edp$. At the start of the proof set $\I=\N$, and let $\widetilde{\Fc}\in K$ be the $\forecaster$ that is nominated to be the $\minimal$ $\forecaster$. We have two cases to consider:    
	\begin{enumerate}
		\item
		For every $\Fc'\in K$, there exists a $\finite$ subset $\cS\subseteq\I$ such that for every $\pk\in (\I \setminus \cS)$ we have $V(\Fc_{\pk}')\ge V(\widetilde{\Fc_{\pk}})-\mu$. In this case we are finished and $\widetilde{\Fc_{\pk}}$ is an $(\mu,\gamma)$-$\minimal$ $\forecaster$ as desired.	
		\item
		There exists $\Fc'\in K$ and $\infinite$ subset $\I'\subseteq \I$ such that for every $\pk\in \I'$ we have $V(\Fc_{\pk}')\le V(\widetilde{\Fc_{\pk}})-\mu$. In this case we set  $\I\leftarrow \I'$, $\widetilde{\Fc} \leftarrow \Fc'$ and reconsider the first case.       
	\end{enumerate}
	
	It remains to justify that this procedure converge and does not continue indefinitely.\\
	By definition every time we replace the nominated $\minimal$ $\forecaster$ (execute the second point) we are guaranteed that $\I$ remains to be of $\infinite$ size, and that for every $n\in\I$ the value of $V(\widetilde{\Fc_{\pk}})$ is reduced by $\mu$.
	Thus we can replace the nominated $\forecaster$ at most $\frac{1}{2\mu}$ times after which the procedure ends, because for every $\pk\in\N$,  and any $\Fc$ ,$0\leq V(\Fc_\pk)\leq 2$.   
\end{proof}


\begin{theorem}[$\oblivious$ $\minimal$ $\forecaster$]
	Let $\eps,\delta,\gamma,\mu>0$ be constants. For every $(\eps,\delta)$-$\EnDpt$ $\edp$,  there exists an \oblivious $(\mu,\gamma)$-$\minimal$ $\forecaster$ $\Fc$ for $\edp$. 
\end{theorem}
\begin{proof}
	In order to prove this theorem we first prove that:
	\begin{claim}
		For every $\gamma$-$\forecaster$ $\Fc$ for $(\eps,\delta)$-$\EnDpt$ $\edp=\enXYTp$ there exists an $\oblivious$  $\gamma$-$\forecaster$ $\Bc$ for $\edp$ such that for every $\pk\in\N$
		\[ V(\Bc_\pk)\leq V(\Fc_\pk) \]	
	\end{claim}
	\begin{proof}(claim)
		The proof is by reduction from $\Fc_\pk$. For every $\pk\in\N$ such that $\edp_\pk^1=(\XYTpo)$,$\edp_\pk^2=(\XYTpt)$ denote two independent copies $\edp_\pk$. We define $\Bc_\pk^1,\Bc_\pk^2$ to be a \singular $\gamma$-$\forecaster$ such that, for every $t_1,t_2\in\Supp(T_\pk)$, $\Bc_\pk^1(t_1)=\Fc_\pk(t_1,T_\pk^2)_1$ and $\Bc_\pk^2(t_2)=\Fc_\pk(T_\pk^1,t_2)_2$.
		
		And for every $i\in\zo$ we define,
		\[Y(\Bc_\pk^i)=\Ex[(X_\pk^i-\Bc_\pk^i(T_\pk^i))^2]\] 
		
		We can now define the $\gamma$-\forecaster $\Bc_\pk'(t_1,t_2)=(\Bc_\pk^1(t_1),\Bc_\pk^2(t_2))$, and by definition $V(\Bc_\pk')=Y(\Bc_\pk^1)+Y(\Bc_\pk^2)$, thus we get that $V(\Bc')= V(\Fc)$ since
		\begin{align*} 
		V(\Fc)&=\Ex[(X_\pk^1-\Fc_\pk(T_\pk^1,T_\pk^2)_1)^2+(X_\pk^2-\Fc_\pk(T_\pk^1,T_\pk^2)_2)^2]\\
		&=\Ex[(X_\pk^1-\Fc_\pk(T_\pk^1,T_\pk^2)_1)^2]+\Ex[(X_\pk^2-\Fc_\pk(T_\pk^1,T_\pk^2)_2)^2]\\
		&= Y(\Bc_\pk^1)+Y(\Bc_\pk^2).\\
		\end{align*}	
		Yet we are not finished, as $\Bc'_\pk$ is not \oblivious. Assume without loss of generality that  $Y(\Bc_\pk^1) \leq Y(\Bc_\pk^2)$ then we define $\Bc_\pk^{\prime\prime}(t_1,t_2)=(\Bc_\pk^1(t_1),\Bc_\pk^{1}(t_2))$ thus 
		\[ V(\Bc_\pk^{\prime\prime})\leq V(\Bc_{\pk}')= V(\Fc_\pk) \]	
		and since $\Bc_\pk^{\prime\prime}$ is \oblivious this concludes the proof.     	
	\end{proof}		
	The theorem follows from lemma \ref{lemma:minimal-forecaster} and the above claim.  	
\end{proof}



%\begin{lemma}[The range of a minimal \forecaster]
%	\label{lemma:range-minimal-eval}
%	Let $\eps,\delta,\gamma,\mu>0$ be constants. and let $\Fc$ be $(\mu,\gamma)$-$\minimal$ $\forecaster$ for $(\eps,\delta)$-$\EnDpt$ $\edp=\set{Z_\pk\eqdef(\XYTp)}_{\pk\in\N}$ with respect to the \infinite set $\I\in\N$. Let $\range$ denote the range $[\half-3\eps,\half+3\eps]$, then the following holds for every $\pk\in\I$:
%	$$
%	\pr{\Fc(T_\pk^1,T_\pk^2)\in\big(\range,\range\big)}>1-something.
%	$$ 
%\end{lemma}

%\begin{proof}(claim)
%The proof will show that if the above is not true, then there exists a more "\minimal" \forecaster, contradicting the minimality of $\Fc$.

%Assume for contradiction that the lemma does not hold, we will define $\gamma$-$\forecaster$ $\Fc'$ such that for every $\pk\in\I$  $V(\Fc_\pk)-V(\Fc'_\pk)>\mu$, thus contradicting the minimality of $\Fc$.

% For every $\pk\in\I$ let $Z^1=(\XYTpo)$ and $Z^2=(\XYTpt)$ denote two independent copies of $Z\pk$, and let $(P_1,P_2)=\Fc(T^1_\pk,T^2_\pk)$, we define $\Fc'_\pk$ as follows:
 
% \[\Fc'_\pk(T^1_\pk,T^2_\pk)= \left\{ \begin{array}{ll}
% (P_1,P_2) & \mbox{if }\\
% 0 & \mbox{otherwise }
% \end{array} \right. \]
 
% \jnote{Work in progress...}
%\end{proof}	




\subsection{Existence of a Good $p^\ast$}

\begin{definition}
	\label{Def:GoodForcast}
	Let $\eps,\gamma,\delta>0$ be constants, and let $\Fc$ be a $\gamma$-\forecaster for the $(\eps,\gamma)$-$\EnDpt$ $\edp=\set{\edp_\pk}_{\pk\in\N}$. For every $\pk\in\N$, we say that $p^{\ast}_\pk\in W_\gamma$ is {\sf a \GoodForecast} with respect to $\Fc_\pk$ and $\edp_\pk$ if the following holds:
	\begin{enumerate}
		\item $p^\ast\notin\zo$.
		\item $\pr{\Fc_\pk(T_\pk^1,T_\pk^2)=(p^\ast,p^\ast)}> (\frac{\gamma\delta}{2})^2$.
		\item $\pr{X_\pk^1=Y_\pk^2| \Fc_\pk(T_\pk^1,T_\pk^2)=(p^\ast,p^\ast)\cap X_\pk^1\ne X_\pk^2}\ge \half+\frac{\delta}{2}-8\eps^2$.
	\end{enumerate}
	Where $\edp_\pk^1=(\XYTpo)$ and $\edp_\pk^2=(\XYTpt)$ denote two independent copies of $\edp_\pk$.

\end{definition}


\begin{lemma}
	Let $\eps,\gamma,\delta>0$ be constants, and let $\Fc$ be a $\gamma$-\forecaster for the $(\eps,\gamma)$-$\EnDpt$ $\edp=\set{\edp_\pk}_{\pk\in\N}$. For every $\pk\in\N$, there exists a {\sf\GoodForecast} $p^{\ast}_\pk\in W_\gamma$ with respect to $\Fc_\pk$ and $\edp_\pk$.
\end{lemma}
\begin{proof}
	ssooooooooooooon.\jnote{Finish this....}
\end{proof}







\begin{lemma}[The range of an \oblivious  \forecaster]
	\label{lemma:range-minimal-forecaster}
	Let $\eps,\delta,\gamma>0$ be constants, and $\Fc$ be an \oblivious $\gamma$-$\forecaster$ for $(\eps,\delta)$-$\EnDpt$ $\edp=\set{Z_\pk\eqdef(\XYTp)}_{\pk\in\N}$. Let $\range$ denote the range $\big([0,\half-3\eps]\cup[\half+3\eps,1]\big)$, then there exists an \oblivious $\gamma$-\forecaster $\Fc'$ such that for every sufficiently large $\pk\in\N$ we have that:
	\begin{enumerate}
		\item $V(\Fc'_\pk)\leq V(\Fc_\pk)$
		\item $\pr{\Fc'_\pk(T_\pk^1,T_\pk^2)=(p',p')}<something(\pk)$ for every $p'\in\cW_\gamma\cap\range$.
	\end{enumerate}
	where $Z^1=(\XYTpo)$ and $Z^2=(\XYTpt)$ denote two independent copies of $Z_\pk$.
\end{lemma}

\begin{proof}(lemma)
	Since $\Fc$ is an \oblivious \forecaster, there exists a \singular \forecaster $\Gc$ such that for every $\pk\in\N$, and every $t^1,t^2\in T_\pk$, $\Fc_\pk(t_1,t_2)=(\Gc_\pk(t_1),\Gc_\pk(t_2))$.
	
	Thus we get that 
	$$
	V(\Fc_\pk)=\ex{\cost(\Gc_\pk(T_\pk^1))}+\ex{\cost(\Gc_\pk(T_\pk^2))}=2\cdot\ex{\cost(\Gc_\pk(T_\pk))}
	$$
	and by lemma \ref{lemma:range-minimal-singular-forecaster} we have that there exists a \singular \forecaster $\Gc'_\pk$ for which $\ex{\cost(\Gc'_\pk(T_\pk))} \leq \ex{\cost(\Gc_\pk(T_\pk))}$ and for every $p'\in \cW_\gamma \cap \range$ we have that $\pr{\Gc'_\pk(T_\pk)=p'}<something(\pk)$. We now define the \forecaster $\Fc'_\pk$ as follows, for every  $t^1,t^2\in T_\pk$, $\Fc'_\pk(t_1,t_2)=(\Gc'_\pk(t_1),\Gc'_\pk(t_2))$. It is easy to see that by lemma \ref{lemma:range-minimal-singular-forecaster} the second point in the lemma holds for $\Fc'$. And the first point in the lemma holds to since by definition,  
	$$
	V(\Fc'_\pk) =2\cdot\ex{\cost(\Gc'_\pk(T_\pk))}\leq2\cdot\ex{\cost(\Gc_\pk(T_\pk))}=V(\Fc_\pk)
	$$ 
	and this concludes the proof.
\end{proof}	

	
\begin{lemma}[The range of a \singular  \forecaster]
	\label{lemma:range-minimal-singular-forecaster}
	Let $\eps,\delta,\gamma>0$ be constants, and let $\Fc$ be a \singular $\gamma$-$\forecaster$ for $(\eps,\delta)$-$\EnDpt$ $\edp=\set{Z_\pk\eqdef(\XYTp)}_{\pk\in\N}$, and denote by $\range$ the range $\big([0,\half-3\eps]\cup[\half+3\eps,1]\big)$. Then there exists a \singular $\gamma$-\forecaster $\Fc'$ such that for every sufficiently large $\pk\in\N$ we have that:
	\begin{enumerate}
		\item $ \ex{\cost(X_\pk,\Fc'_\pk(T_\pk))}\leq \ex{\cost(X_\pk,\Fc_\pk(T_\pk))}$
		\item $\pr{\Fc'_\pk(T_\pk)=p}<\something(\pk)$, for every $p\in\cW_\gamma\cap\range$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	Let $\rangeZero$ denote the range $[0,\half-3\eps]$ and $\rangeOne$ denote the range $[\half+3\eps,1]$.	For every $\pk\in\N$, we define the function $C:\cW_\gamma \to [0,1]$ as follows, for every $p\in\cW_\gamma$, $C(p)=\pr{\Fc_\pk(T_\pk)=p}$.
	Let $\cS^0,\cS^1\subset\cW_\gamma$ denote the subset of forecasts that fall in the range $\rangeZero$ and $\rangeOne$, and happen with probability $\something(\pk)$. Namely for every $i\in\zo$
	$$
	\cS^i=\set{p': C(p')>\something(\pk), p'\in\range_i, p'\in\cW_\gamma }.
	$$ 
	For every $\pk\in\N$ the new $\gamma$-$\forecaster$ $\Fc_\pk$ will be defined using the original \forecaster $\Fc_\pk$. For every $t\in \Supp(T_\pk)$: 
	
	
	$$
	\Fc'_\pk(t)= \left\{ \begin{array}{ll}
	\half & \mbox{if $\Fc_\pk(t)\in \cS^0\cup\cS^1$ }\\
	\Fc_\pk(t) & \mbox{otherwise }
	\end{array} \right. 
	$$
	
	By definition, $\Fc'_\pk$ satisfies the second point in the lemma. Let $B=\set{\Fc_\pk(T_\pk)\in\cS^0\cup\cS^1}$ be a random event, and observe that $ \ex{\cost(X_\pk,\Fc'_\pk(T_\pk)|\overline{B})}= \ex{\cost(X_\pk,\Fc_\pk(T_\pk))|\overline{B}}$ since  $\Fc_\pk$ and  $\Fc'_\pk$ have the same output when conditions on the event $\overline{B}$. And from claim \ref{claim:range-singular-forecaster} we have that $ \ex{\cost(X_\pk,\Fc'_\pk(T_\pk)|B)}\le \ex{\cost(X_\pk,\Fc_\pk(T_\pk))|B}$, this means that the first point in the lemma also holds, and this concludes the proof. 
\end{proof}


\begin{claim}
	\label{claim:range-singular-forecaster}
	Let $\eps,\delta,\gamma>0$ be constants, and let $\Fc$ be a \singular $\gamma$-$\forecaster$ for $(\eps,\delta)$-$\EnDpt$ $\edp=\set{Z_\pk\eqdef(\XYTp)}_{\pk\in\N}$. For every $\pk\in\N$ and fixed $p'\in\big([0,\half-3\eps]\cup[\half+3\eps,1]\big)$ such that $\pr{\Fc_\pk(T_\pk)=p'}>\something(\pk)$, it holds that $\ex{\cost(X_\pk,\Fc_\pk(T_\pk))|\Fc_\pk(T_\pk)=p'}\ge\frac{1}{4}$.
\end{claim}
\begin{proof}
		For every $\pk\in\N$ what follows holds true. For every $p'$ that is considered in the claim, we define the \ppt $\Dc_\pk$ as follows, for every $t\in\Supp(T_\pk)$,
			$$
			\Dc'_\pk(t)= \left\{ \begin{array}{ll}
			1 & \mbox{if $\Fc_\pk(t)=p'$ }\\
			0 & \mbox{otherwise }
			\end{array} \right. 
			$$
		we now note that by the \dpt properties we get that $\pr{X_\pk=1|\Dc_\pk(1)}=\pr{X_\pk=1|\Fc_\pk(T_\pk)=p'}\in [\half-\eps,\half+\eps]$.
		
		It is easy to see that
			\begin{align*}
			\ex{\cost(X_\pk,\Fc_\pk(T_\pk))|\Fc_\pk(T_\pk)=p'}&=\ex{\cost(X_\pk,p')|\Fc_\pk(T_\pk)=p'}\\
																&=\ex{(X_\pk-p')^2|\Fc_\pk(T_\pk)=p'}\\
																&=\pr{x=1|\Fc_\pk(T_\pk)=p'}\cdot(1-p')^2+\pr{x=1|\Fc_\pk(T_\pk)=p'}\cdot (p')^2\\
																&=\pr{x=1|\Fc_\pk(T_\pk)=p'}\cdot(1-2p')+(p')^2.\\
			\end{align*} 
		Let $\half\ge\beta,\alpha\ge-\half$ be constants, such that $p'=\half+\beta$ and  $\pr{X_\pk=1|\Fc_\pk(T_\pk)=p'}=\half+\alpha$, and we get that:
		\begin{align*}
		\ex{\cost(X_\pk,\Fc_\pk(T_\pk))|\Fc_\pk(T_\pk)=p'}&=(\half+\alpha)\cdot(1-2(\half+\beta))+(\half+\beta)^2\\
														  &=\frac{1}{4}+\beta^2 -2\alpha\beta >\frac{1}{4} \\									  
		\end{align*}
		where that last inequality follows because in our setting, namely  $\alpha\in[-\eps,+\eps]$ and $\beta\in\big([-\half,-3\eps]\cup[3\eps,\half]\big)$, we have that the inequality $\beta^2>2\alpha\beta$ always holds true. 
	
\end{proof}



\begin{lemma}
	\label{lemma:p-with-x1!x2}
		Given an \oblivious $\gamma$-\forecaster $\Fc$ for the two independent copies of the $(\eps,\delta)$-\dpt $Z_1=(X_1,Y_1,T_1)$ and $Z_2=(X_2,Y_2,T_2)$. Let $\Fc(T_1,T_2)=(P_1,P_2)$ then there exists $p^\ast\in \cW_\gamma$ such that:
	\begin{enumerate}
		\item $\pr{P_1=P_2=p^\ast}> (\frac{\gamma\delta}{2})^2$,
		\item $\pr{X_1=Y_1| P_1=P_2=p^\ast, X_1\ne X_2}\ge \half+\frac{\delta}{2}-8\eps^2$.
	\end{enumerate}  
\end{lemma}
\begin{proof}
	By lemma \ref{lemma:good-p} there exists $p^\ast\in \cW_\gamma$ such that $\Pr[P_1=P_2=p^\ast]> (\frac{\gamma\delta}{2})^2$ and $\Pr[X_1=Y_1| P_1=P_2=p^\ast]\ge \half+\frac{\delta}{2}$.\\
	\jnote{This claim/lemma needs more work (a lot), we need to deal with the computational aspect, from my calculations this should be true, I'll do this later after we agree on the definitions for the computational model}
	\begin{claim}
		For every $p^\ast\in \cW_\gamma$ such that $\Pr[X_1=Y_1| P_1=P_2=p^\ast]\ge \half+\frac{\delta}{2}$, it holds that $\Pr[X_1=Y_1| P_1=P_2=p^\ast,X_1\ne X_2]\ge \half+\frac{\delta}{2}-8\eps^2$  
	\end{claim}
	
	\begin{proof}(claim)
		Let $B$ denote a random event such that $B=\{P_1=P_2=p^\ast\}$. We will compare $\Pr[X_1=Y_1| B]$ and $\Pr[X_1=Y_1| B\cap(X_1\ne X_2)]$, and show that by the $\mech$  properties the two probabilities are close.  

		We denote $\alpha_1=\Pr[X_1=Y_1|X_1=1\cap B]$ and $\alpha_0=\Pr[X_1=Y_1|X_1=0\cap B]$ by definition we have that
		\begin{align*}
		\Pr[X_1=Y_1|B]&=\Pr[X_1=Y_1|X_1=1\cap B]\cdot\Pr[X_1=1|B]+\Pr[X_1=Y_1| X_1=0\cap B]\cdot\Pr[X_1=0|B]\\
					&=\alpha_1\cdot\Pr[X_1=1|B]+\alpha_0\cdot\Pr[X_1=0|B],\\
					&\leq \half(\alpha_1+\alpha_0)+2\eps^2
		\end{align*}
		since by the $\mech$ properties we know that $\alpha_1,\alpha_2\in [\half - \eps,\half+\eps]$ and $\Pr[X_1=1|B]\in [\half - \eps,\half+\eps]$.
		And on the other hand we have that 
		\[ \Pr[X_1=Y_1| B\cap(X_1\ne X_2)]=\alpha_1\cdot\Pr[X_1=1|B\cap(X_1\ne X_2)]+\alpha_0\cdot\Pr[X_1=0|B\cap(X_1\ne X_2)],\]		
		where this equality follows because for every $i\in\zo$ 
		\[ \alpha_i=\Pr[X_1=Y_1|X_1=i\cap B]=\Pr[X_1=Y_1|X_1=i\cap B\cap(X_1\ne X_2)].\]
		
		We stress that the conditioning on $X_1\ne X_2$ still gives us a bounded probability, and we get\footnote{We can do much better..}: 
		\[\Pr[X_1=1|B\cap(X_1\ne X_2)]\in [\half - 3\eps,\half+3\eps]\]
		thus we get that 
		\[\Pr[X_1=Y_1| B\cap(X_1\ne X_2)]\geq\half(\alpha_1+\alpha_0)-6\eps^2.\]  
		 Recall that by assumption we have that $\Pr[X_1=Y_1|B]\geq\half+\frac{\delta}{2}$ this means that $\Pr[X_1=1|B\cap(X_1\ne X_2)]\geq\half+\frac{\delta}{2}-8\eps^2$ as desired, where that last inequality follows since
		  $\Pr[X_1=Y_1| B]-\Pr[X_1=Y_1| B\cap(X_1\ne X_2)]\leq 8\eps^2$, thus the proof holds.  
%		 Let $p^\ast\in \cW_\gamma$ be as assumed in that claim, and denote $\alpha_0=\Pr[Y_1=0|P_1=P_2=p^\ast,X_1=0]$ and $\alpha_1=\Pr[Y_1=1|P_1=P_2=p^\ast,X_1=1]$. We first observe that by the assumption:
%		 \[\Pr[X_1=Y_1|P_1=P_2=p^\ast]=\alpha_0\cdot\Pr[X_1=0|P_1=P_2=p^\ast]+\alpha_1\cdot\Pr[X_1=1|P_1=P_2=p^\ast]\]
%But we also have that:
%		 	  	\begin{align*}
%		 	  \Pr[X_1=Y_1|P_1=P_2=p^\ast,X_1\ne X_2]=&\alpha_0\cdot\Pr[X_1=0|P_1=P_2=p^\ast,X_1\ne X_2]\\
%		 	  &+\alpha_1\cdot\Pr[X_1=1|P_1=P_2=p^\ast,X_1\ne X_2]
%		 	  	\end{align*}
%this is true because $\alpha_0=\Pr[Y_1=0|P_1=P_2=p^\ast,X_1=0]=\Pr[Y_1=0|P_1=P_2=p^\ast,X_1=0,X_2=1]$ and $\alpha_1=\Pr[Y_1=1|P_1=P_2=p^\ast,X_1=1]=\Pr[Y_1=1|P_1=P_2=p^\ast,X_1=1,X_2=0]$, but note that by assumption (we have yet to justify, need to do that later),  $\alpha_1,\alpha_0\in [\half - \eps,\half+\eps]$, and $\Pr[X_1=0|P_1=P_2=p^\ast,X_1\ne X_2],\Pr[X_1=1|P_1=P_2=p^\ast,X_1\ne X_2]\in [\half - \eps,\half+\eps]$

%This means that $\Pr[X_1=Y_1|P_1=P_2=p^\ast,X_1\ne X_2]\leq\half+\frac{\delta}{2}-4\eps^2$.       		 	  	
	\end{proof}	 
	The proof follows from the claim.
\end{proof}


\begin{lemma}
	\label{lemma:good-p}
	Given an \oblivious $\gamma$-\forecaster $\Fc$ for the two independent copies of the $(\eps,\delta)$-\dpt $Z_1=(X_1,Y_1,T_1)$ and $Z_2=(X_2,Y_2,T_2)$. Let $\Fc(T_1,T_2)=(P_1,P_2)$ then there exists $p^\ast\in \cW_\gamma$ such that:
	\begin{enumerate}
		\item $\pr{P_1=P_2=p^\ast}\geq (\frac{\gamma\delta}{2})^2$,
		\item $\pr{X_1=Y_1| P_1=P_2=p^\ast}\ge \half+\frac{\delta}{2}$.
	\end{enumerate}  
	
\end{lemma}
\begin{proof}
	The proof will first show that:	
	%We assume for contradiction that there exists no $p^\ast\in \cW$ such that the above holds.
	\begin{claim}
		\label{Claim-p1}
		There exists $p^\ast\in \cW_\gamma$ such that $\Pr[P_1=p^\ast]\geq (\frac{\gamma\delta}{2})$ and it holds that $\Pr[X_1=Y_1| P_1=p^\ast]\ge \half+\frac{\delta}{2}$. 
	\end{claim}
	\begin{proof}(claim)
		Assume for contradiction that there does not exists $p^\ast\in \cW_\gamma$ such that the claim holds, and define function $C:\cW_\gamma\rightarrow[0,1]$ such that for every $p'\in \cW_\gamma$, $C(p')=\Pr[P_1=p']$.
		
		Let $\cD=\set{p'|C(p')<\frac{\gamma\delta}{2} ,p'\in \cW_\gamma}$ denote the set of all possible results for $P_1$ that appears with probability less than $\frac{\gamma\delta}{2}$,  since $|\cW_\gamma|<\floor{\frac{1}{\gamma}}$ we have that
		\[ \Pr[P_1\in \cD]< |\cW_\gamma|\cdot\frac{\gamma\delta}{2}<\frac{\delta}{2}.\]
		
		Note that by the assumption $\Pr[X_1=Y_1|P_1\notin \cD]<\half+\frac{\delta}{2}$, and by the $\mech$ property we have that $\Pr[X_1=Y_1]\ge \half+\delta$. But we know that $\Pr[X_1=Y_1]=\Pr[X_1=Y_1|P_1\in \cD]\cdot\Pr[P_1\in \cD]+\Pr[X_1=Y_1|P_1\notin \cD]\cdot\Pr[P_1\notin \cD]<1\cdot\frac{\delta}{2}+(\half+\frac{\delta}{2})\cdot(1-\frac{\delta}{2})<\half+\frac{3\delta}{4}$\footnote{We can get getter better results if we use the DP, the 1/2+$\eps$ bound but it's not really important}, thus we get a contradiction and the claim holds.  	
	\end{proof}	
	
	By obliviousness of $\Fc$ we have that there exists $\Fc'$ such $\Fc(T_1,T_2)=(\Fc'(T_1),\Fc'(T_2))$, this means that $P_1=\Fc'(T_1)$ and $P_2=\Fc'(T_2)$. By claim \ref{Claim-p1} and the obliviousness property there exists $p^\ast\in \cW_\gamma$ that satisfies both points of the lemma since $T_1,T_2$ are independent variables sampled from the same distribution, and the claim holds.
	
\end{proof}



\subsection{Analysis for $\Fc^\ast$}\label{sec:LB:Analyzes}

Here we have the lemmas and claims we used to prove and analyze the improved minimal \forecaster $\Fc^\ast$.

\begin{definition}[Eve]
	\label{def:Charlie}
	Given a $\gamma$-\forecaster $\Fc$ for the two independent copies of the $(\eps,\delta)$-\dpt $Z_1=(X_1,Y_1,T_1)$ and $Z_2=(X_2,Y_2,T_2)$, and  $p^\ast\in\cW_\gamma$. Let $\Fc(T_1,T_2)=(P_1,P_2)$.
	We say that \ppt $\Ec^{\Fc}$ with oracle access to $\Fc$ is an attach that breaks the Protocol (KA) specified by figure-\ref{fig:KA-Protocol} if: 
	\[\Pr[\Ec^{\Fc}(T_1,T_2)=X_1|P_1=P_2=p^\ast,X_1\ne X_2] \ge \frac{1}{2}+\frac{\delta}{4}.\]    
\end{definition}



\begin{algorithm}[Algorithm $\Fc^\ast$]\label{alg:improve}
	\item[Parameter:] $\gamma$ and $p^\ast \in \cW_\gamma$.
	
	\item[Input:]  $t_1,t_2\in \Supp(T)$
%	\item[Oracle:] ?
	
	\begin{enumerate}
		\item Let $(p_1,p_2) = \Fc(t_1,t_2) $
		\item If $p_1=p_2=p^\ast$.
		\begin{enumerate}
			\item If $\Ec(t_1,t_2)=1$ output $(p^\ast+ \gamma,p^\ast- \gamma)$
			\item If $\Ec(t_1,t_2)=0$ output $(p^\ast- \gamma,p^\ast+ \gamma)$	
		\end{enumerate}
		Else, output $(p_1,p_2)$.
	\end{enumerate}
	
\end{algorithm}




\begin{lemma}
	Given an \oblivious $\gamma$-\forecaster $\Fc$ for the two independent copies of the $(\eps,\delta)$-\dpt $Z_1=(X_1,Y_1,T_1)$ and $Z_2=(X_2,Y_2,T_2)$, there does not exist a \ppt $\Ec^\Fc$ that breaks the KA Protocol specified by $\Fc$ and the good $p^\ast$ that is garmented by lemma \ref{lemma:p-with-x1!x2}.       
\end{lemma}
\begin{proof}
	The proof will proceed by showing that if an attack $\Ec^\Fc$ does indeed exist then this implies that $\Fc$ is not a $(\mu,\gamma)$-minimal \forecaster. We prove this by reduction from $\Ec^\Fc$, constructing a $\gamma$-\forecaster $\Fc^\ast$ that contradicts the minimality of $\Fc$.
	
	Given $\Fc$, assume for contradiction that an attack $\Ec^\Fc$ exists and let $\Fc^\ast$ be as defined \ref{alg:improve} with $p^\ast\in\cW_\gamma$ that is guaranteed by lemma \ref{lemma:p-with-x1!x2}, we will show that $V(\Fc)-V(\Fc^\ast)>\mu$ thus contradicting the minimality of $\Fc$.
	
	Let us now analyze $V(\Fc^\ast)$ and compare it to $V(\Fc)$, we define the random event $B=\{\Fc(T_1,T_2)=(p^\ast,p^\ast)\}$, recall that:
	\[V(\Fc)=\Pr[B]\cdot V(\Fc|B)+\Pr[\overline{B}]\cdot V(\Fc|\overline{B})\]	
	By definition we have that $V(\Fc|\overline{B})=V(\Fc^\ast|\overline{B})$ since $\Fc^\ast$ and $\Fc$ have that same output whenever $\Fc(T_1,T_2)\ne(p^\ast,p^\ast)$, thus we get that:
	\begin{align*}
	V(\Fc)-V(\Fc^\ast)&=\Pr[B]\cdot(V(\Fc|B)-V(\Fc^\ast|B))+\Pr[\overline{B}]\cdot(V(\Fc|\overline{B})-V(\Fc^\ast|\overline{B}))\\
	&=\Pr[B]\cdot(V(\Fc|B)-V(\Fc^\ast|B))\\
	&<(\frac{\gamma\delta}{2})^2\cdot(\frac{\delta\gamma}{2}-2\gamma^2-\eps\gamma\delta)
	\end{align*}
	where the last inequality follows by lemma \ref{lemma:p-with-x1!x2} that states that $\Pr[B]>(\frac{\gamma\delta}{2})^2$, and by lemma \ref{lemma:cond-gain} that shows that $(V(\Fc|B)-V(\Fc^\ast|B))>(\frac{\delta\gamma}{2}-2\gamma^2-\eps\gamma\delta)$.
	
	
	This concludes the proof since ... 
\end{proof}


\begin{lemma}
	\label{lemma:cond-gain}
	Given an \oblivious $\gamma$-\forecaster $\Fc$ for the two independent copies of the $(\eps,\delta)$-\dpt $Z_1=(X_1,Y_1,T_1)$ and $Z_2=(X_2,Y_2,T_2)$, $p^\ast\in \cW_\gamma$ as guaranteed by lemma \ref{lemma:p-with-x1!x2}  and an attack $\Ec^\Fc$. Let $\Fc^\ast$ be defined by specified by $\ref*{alg:improve}$ for $\Fc$, $p^\ast$ and $\Ec^\Fc$, then  
	\[V(\Fc|B)-V(\Fc^\ast|B)>\frac{\delta\gamma}{2}-2\gamma^2-\eps\gamma\delta\]
	where $B=\{\Fc(T_1,T_2)=(p^\ast,p^\ast)\}$. 
\end{lemma}
\begin{proof}
	The proof will partition the analyzes into two cases, conditioned on the relationship between $X_1,X_2$. We define the two random events $B_{eq}=B\cap \{X_1=X_2\}$ and $B_{neq}=B\cap \{X_1\ne X_2\}$, and denote,
		\begin{enumerate}
			\item $Y_{eq}=V(\Fc|B_{eq})-V(\Fc^\ast|B_{eq})$,  
			\item $Y_{neq}=V(\Fc|B_{neq})-V(\Fc^\ast|B_{neq})$.	
		\end{enumerate}
	Hence we get that,	 
	\[V(\Fc|B)-V(\Fc^\ast|B)= \Pr[B_{eq}|B]\cdot Y_{eq}+ \Pr[B_{neq}|B]\cdot Y_{neq}\]

	From claim \ref{claim:eq-event}, we have that $Y_{eq}=-2\gamma^2$, and from claim \ref{claim:not-eq-event} we have that $Y_{neq}=\gamma\delta-2\gamma^2$. to conclude the proof note that by the definition of the $\mech$ \footnote{This is not accurate, this should be changed when we agree on the actual bound for the computational DP, but the real value should not be far from this calculation.} $\Pr[B_{eq}|B]\leq \half+\eps$, thus we get:
\begin{align*}
	V(\Fc|B)-V(\Fc^\ast|B)&\geq (\half+\eps)\cdot (-2\gamma^2)+ (\half-\eps)\cdot (\gamma\delta-2\gamma^2)\\
						&\geq\frac{\delta\gamma}{2}-2\gamma^2-\eps\gamma\delta
\end{align*}	 	
\end{proof}


\begin{claim}
		\label{claim:not-eq-event}
			Given an \oblivious $\gamma$-\forecaster $\Fc$ for the two independent copies of the $(\eps,\delta)$-\dpt $Z_1=(X_1,Y_1,T_1)$ and $Z_2=(X_2,Y_2,T_2)$, $p^\ast\in \cW_\gamma$ as guaranteed by lemma \ref{lemma:p-with-x1!x2} and an attack $\Ec^\Fc$. Let $\Fc^\ast$ be defined by $\Fc$, $p^\ast$ and $\Ec^\Fc$. We define the random event $B_{neq}=\{\Fc(T_1,T_2)=(p^\ast,p^\ast)\cap X_1\ne X_2\}$ then it holds that
		\[V(\Fc|B_{neq})-V(\Fc^\ast|B_{neq})=\gamma\delta-2\gamma^2 \]
\end{claim}
\begin{proof}
	The main observation in this proof is that the conditioning on $B_{neq}$ creates the exact probability space that is considered in the attach $\Ec^\Fc$.   
	For the analysis we will consider two cases conditioned on the success or failure of the attach $\Ec^\Fc$, and define the two random evens:
	\begin{itemize}
		\item $B_{hit}=B_{neq}\cap\{\Ec^\Fc(T_1,T_2)=X_1\}$,
		\item $B_{miss}=B_{neq}\cap\{\Ec^\Fc(T_1,T_2)\ne X_1\}$
	\end{itemize}
we will examen the lose and gain for conditioning on the event $B_{hit}$, and we denote it by $Y_{hit}=V(\Fc|B_{hit})-V(\Fc^\ast|B_{hit})$, by definition we have
	 \begin{align*}
	  Y_{hit}&=\Ex[\price_{\Fc}(X_1,X_2,T_1,T_2)|B_{hit}]-\Ex[\price_{\Fc^\ast}(X_1,X_2,T_1,T_2)|B_{hit}]\\
	 &=\Ex[\price_{\Fc}(X_1,X_2,T_1,T_2)-\price_{\Fc^\ast}(X_1,X_2,T_1,T_2)|B_{hit}]\\
	 &=2\gamma-2\gamma^2
	 \end{align*}
	 	where the last equality follows from claim \ref{claim:hit-or-mis} first point, since for every fixing of $X_1=x_1$, $X_2=x_2$, $T_1=t_1$ and $T_2=t_2$ such that $x_1 \ne x_2$, $\Ec^\Fc(t_1,t_2)=x_1$ and $\Fc(t_1,t_2)=(p^\ast,p^\ast)$ we get that $\price_{\Fc}(x_1,x_2,t_1,t_2)-\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)=2\gamma-2\gamma^2$.
	 	
	 	Similarly when we condition on the event $B_{miss}$ and denote $Y_{miss}=V(\Fc|B_{miss})-V(\Fc^\ast|B_{miss})$, by definition we have
	 	\begin{align*}
	 	Y_{miss}&=\Ex[\price_{\Fc}(X_1,X_2,T_1,T_2)|B_{miss}]-\Ex[\price_{\Fc^\ast}(X_1,X_2,T_1,T_2)|B_{miss}]\\
	 	&=\Ex[\price_{\Fc}(X_1,X_2,T_1,T_2)-\price_{\Fc^\ast}(X_1,X_2,T_1,T_2)|B_{miss}]\\
	 	&=-2\gamma-2\gamma^2
	 	\end{align*}
	 	Here the last equality follows from claim \ref{claim:hit-or-mis} second point, since for every fixing of $X_1=x_1$, $X_2=x_2$, $T_1=t_1$ and $T_2=t_2$ such that $x_1 \ne x_2$, $\Ec^\Fc(t_1,t_2)\ne x_1$ and $\Fc(t_1,t_2)=(p^\ast,p^\ast)$ we get that $\price_{\Fc}(x_1,x_2,t_1,t_2)-\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)=-2\gamma-2\gamma^2$.
	 	
	 	
	 	Finally to conclude the proof note that
	 	\begin{align*}
	 	V(\Fc|B_{neq})-V(\Fc^\ast|B_{neq})&=\Pr[B_{hit}|B_{neq}]\cdot Y_{hit}+\Pr[B_{miss}|B_{neq}] \cdot Y_{miss}\\
									 &\geq(\frac{1}{2}+\frac{\delta}{4})\cdot Y_{hit}+\geq(\frac{1}{2}-\frac{\delta}{4})\cdot Y_{miss}\\
									 &\geq(\frac{1}{2}+\frac{\delta}{4})\cdot(2\gamma-2\gamma^2)+(\frac{1}{2}-\frac{\delta}{4})\cdot(-2\gamma-2\gamma^2)\\
									 &\geq \delta\gamma -2\gamma^2
	 \end{align*}
	 Where the second equality follows by the definition of the attach $\Ec^\Fc$, and we have that 
	 	\[\Pr[B_{hit}|B_{neq}]=\Pr[\Ec^{\Fc}(T_1,T_2)=X_1|\Fc(T_1,T_2)=(p^\ast,p^\ast),X_1\ne X_2] \ge \frac{1}{2}+\frac{\delta}{4}\]
	 	and the claim holds.  
\end{proof}

\begin{claim}[price difference for $X_1\ne X_2$]
	\label{claim:hit-or-mis}
	Let  $\Fc$ be an \oblivious $\gamma$-\forecaster for a $(\eps,\delta)$-\dpt $Z=(\XYT)$. For a fixed $p^\ast\in \cW_\gamma$, let $\Ec^\Fc$ to be an attack as stated in \ref{def:Charlie}, and define $\Fc^\ast$ according to \ref{alg:improve}. The following holds, for every  $x_1,x_2\in \Supp (X)$,$t_1,t_2\in \Supp(T)$ such that $x_1\ne x_2$ and $\Fc(t_1,t_2)=(p^\ast,p^\ast)$: if $\Ec^\Fc(t_1,t_2)=x_1$ then $\price_{\Fc}(x_1,x_2,t_1,t_2)-\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)=2\gamma-2\gamma^2$. Else, if $\Ec^\Fc(t_1,t_2)\ne x_1$, then 
		$\price_{\Fc}(x_1,x_2,t_1,t_2)-\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)=-2\gamma-2\gamma^2$.
\end{claim}
\begin{proof}
	By definition for a fixed $x_1\ne x_2$ we have that,
	\[ \price_{\Fc}(x,x,t_1,t_2)=(1-p^\ast)^2+(p^\ast)^2\]
	and recall that this setting where $\Fc(t_1,t_2)=(p^\ast,p^\ast)$ is exactly the place where the output $\Fc^\ast$ differs from $\Fc$, and so we have two cases, if $\Ec^\Fc(t_1,t_2)=x_1$ then:    
	\[ \price_{\Fc^\ast}(x,x,t_1,t_2)=(1-p^\ast-\gamma)^2+(p^\ast-\gamma)^2=(1-p^\ast)^2+(p^\ast)^2-2\gamma+2\gamma^2\]
	here we point out that the output of $\Fc^\ast$ was changed from $(p^\ast,p^\ast)$ to either $(p^\ast+\gamma,p^\ast-\gamma)$ if $\Ec^\Fc(t_1,t_2)=x_1=1$ or to $(p^\ast-\gamma,p^\ast+\gamma)$ if $\Ec^\Fc(t_1,t_2)=x_1=0$, but in either case the value of $\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)$ remains the same.
	As for the second case, if $\Ec^\Fc(t_1,t_2)\ne x_1$ then:
	\[ \price_{\Fc^\ast}(x,x,t_1,t_2)=(1-p^\ast+\gamma)^2+(p^\ast+\gamma)^2=(1-p^\ast)^2+(p^\ast)^2+2\gamma+2\gamma^2\]
	 here too we point out that the output of $\Fc^\ast$ was changed from $(p^\ast,p^\ast)$ to either $(p^\ast+\gamma,p^\ast-\gamma)$ if $\Ec^\Fc(t_1,t_2)\ne x_1=1$ or to $(p^\ast-\gamma,p^\ast+\gamma)$ if $\Ec^\Fc(t_1,t_2)\ne x_1=0$, but in either case the value of $\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)$ remains the same.
	   
	   
	By the calculations above, it is easy to see that the claim holds.
\end{proof}


\begin{claim}
	\label{claim:eq-event}
		Given an \oblivious $\gamma$-\forecaster $\Fc$ for $\mech$ $\edp$, $p^\ast\in \cW_\gamma$ and an attack $\Ec^\Fc$ \Inote{Unclear. Algorithm?}. Let $\Fc^\ast$ be defined by $\Fc$, $p^\ast$ and $\Ec^\Fc$, and define the random event $B_{eq}=\{A(T_1,T_2)=(p^\ast,p^\ast)\cap X_1=X_2\}$ then it holds that
	\[V(\Fc|B_{eq})-V(\Fc^\ast|B_{eq})=-2\gamma^2 \]
\end{claim}	 \Inote{Same comments as above}
\begin{proof}
By definition we have that
	
	 \begin{align*}
		 V(\Fc|B_{eq})-V(\Fc^\ast|B_{eq})&=\Ex[\price_{\Fc}(X_1,X_2,T_1,T_2)|B_{eq}]-\Ex[\price_{\Fc^\ast}(X_1,X_2,T_1,T_2)|B_{eq}]\\
										&=\Ex[\price_{\Fc}(X_1,X_2,T_1,T_2)-\price_{\Fc^\ast}(X_1,X_2,T_1,T_2)|B_{eq}]\\
										&=-2\gamma^2
	 \end{align*}

	where the last equality follows from claim \ref{claim:diff-11}, since for every fixing of $X_1=x_1$, $X_2=x_2$, $T_1=t_1$ and $T_2=t_2$ such that $x_1=x_2$ and $\Fc(t_1,t_2)=(p^\ast,p^\ast)$ we get that $\price_{\Fc}(x_1,x_2,t_1,t_2)-\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)=-2\gamma^2$, and thus the claim holds. 
\end{proof}



	Given an \oblivious $\gamma$-\forecaster $\Fc$ for the two independent copies of the $(\eps,\delta)$-\dpt $Z_1=(X_1,Y_1,T_1)$ and $Z_2=(X_2,Y_2,T_2)$, $p^\ast\in \cW_\gamma$ as guaranteed by lemma \ref{lemma:p-with-x1!x2} and an attack $\Ec^\Fc$. Let $\Fc^\ast$ be defined by $\Fc$, $p^\ast$ and $\Ec^\Fc$.

\begin{claim}(false difference for $X_1=X_2$)
	\label{claim:diff-11}
	Given an \oblivious $\gamma$-\forecaster $\Fc$ for $\mech$ $\edp$, $p^\ast\in \cW_\gamma$ and an attack $\Ec^\Fc$. Let $\Fc^\ast$ be defined by $\Fc$, $p^\ast$ and $\Ec^\Fc$. For every fixed $x_1,x_2,t_1,t_2$ such that $x_1=x_2$ and $\Fc(t_1,t_2)=(p^\ast,p^\ast)$
	\[ \price_{\Fc}(x_1,x_2,t_1,t_2)-\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)=-2\gamma^2 \] 
\end{claim}
\begin{proof}
	By definition for a fixed $x_1=x_2=x$ we have that,
	\[ \price_{\Fc}(x,x,t_1,t_2)=(x-p^\ast)^2+(x-p^\ast)^2=2(x-p^\ast)^2 \]
	and recall that this setting where $\Fc(t_1,t_2)=(p^\ast,p^\ast)$ is exactly the place where the output $\Fc^\ast$ differs from $\Fc$, and we get:    
	\[ \price_{\Fc^\ast}(x,x,t_1,t_2)=(x-p^\ast+\gamma)^2+(x-p^\ast-\gamma)^2=2(x-p^\ast)^2+2\gamma^2\]
	here we point out that the output of $\Fc^\ast$ was changed from $(p^\ast,p^\ast)$ to either $(p^\ast+\gamma,p^\ast-\gamma)$ or $(p^\ast-\gamma,p^\ast+\gamma)$ depending on the output of $E^{\Fc}$, but in either case the value of $\price_{\Fc^\ast}(x,x,t_1,t_2)$ remains the same. 
	Thus we get that:	
	\[ \price_{\Fc}(x_1,x_2,t_1,t_2)-\price_{\Fc^\ast}(x_1,x_2,t_1,t_2)=-\gamma^2 \]
	and the claim hold.
\end{proof}







==> overview.tex <==
\section{Proof Overview}\label{sec:overview}
In this section we give a high level informal overview of the proof of \cref{thm:mainInf}. The purpose of this section is to outline the proof technique, point out some of the main challenges, and explain how we overcome them. We will allow ourselves to be informal and imprecise. The actual proof appears in the technical part of the paper, and does not build on this section. The reader can skip to the formal section at any time. In the text below we use footnotes to comment on issues where the informal outline is oversimplified compared to the actual proof.

\smallskip
 Let $\Pi = (\Ac,\Bc)$ be a protocol, and consider $\Pi(1^\kappa) =(\Ac,\Bc)(1^\kappa)=(X_\kappa,Y_\kappa,T_\kappa)$. From now on, to avoid clutter, we will omit $\kappa$ whenever it is clear from the context.

 Our goal is to understand the ``correlation between $X$ and $Y$ from the point of view of a \pptm  $\Ec$ that receives $T$ as input''. In this overview, we will mostly ignore $Y$ and ask ``what does $\Ec$ know about $X$''. This is already sufficient to demonstrate some of the main ideas in this paper, and the framework explained in \cref{sec:intro:Technique}.

 \subsection{(Partial) Forecasters}

 We set up a competition between all poly-time machines. (Let us oversimplify and assume that we only consider deterministic polynomial time machines $\Fc$).\footnote{A significant part of the technical work in this paper is devoted to showing that it is sufficient to deal with deterministic machines in order to handle randomized machines. We do not go into such details in this informal overview.} We call such machines forecasters.\footnote{Actually, later on we will set a more advanced competition that also involves $Y$, and so in the technical part, the participants of the current competition are called ``partial forecasters''.}
 For every forecaster $\Fc$ (and choice of $\kappa$) we associate a price, $\Price_{\kappa}(\Fc) \in [0,1]$. The goal of a forecaster is to pay the smallest possible price.

 \subsubsection{Existence of Optimal Forecasters}

 The choice of the price function plays an important role in this paper, and we will soon discuss it. However, for every price function this competition has winners, in the following sense: we say that $\Fc$ is {\sf $\mu$-optimal}, if exists infinite subset $ \II \subseteq \N$ such that  $\Price_{\kappa}(\Fc) \le \Price_{\kappa}(\Fc') + \mu$ for every other forecaster $\Fc'$ and  sufficiently large $\kappa\in \II$. This intuitively says that $\Fc$ cannot be significantly improved on the subset $\II$. We claim that for every constant $\mu>0$ there exists a $\mu$-optimal forecaster.

This is because we can imagine the following iterative process: we start with some forecaster $\Fc$ and $\II=\N$. At each step, either $\Fc$ cannot be improved by $\mu$, on infinitely many $\kappa \in \II$ (which means that $\Fc$ is $\mu$-optimal), or else, there exists an infinite $\II' \subseteq \II$, and a forecaster $\Fc'$ that improves $\Fc$ by $\mu$ in $\II'$. In that case we set $\II=\II'$, $\Fc'=\Fc$ and continue. It is clear that at every iteration we improve the price by $\mu$, and as this can happen only a bounded number of times, this process shows the existence of a $\mu$-optimal forecaster.\footnote{A drawback of the argument above is that it only works for constant $\mu>0$. The distinguishing parameter $\rho$, will be selected to be say $\mu^{1/100}$, and this is why we only get the result in \cref{thm:mainInf} for constant $\rho>0$. Consequently, if we could guarantee the existence of an optimal forecaster for smaller $\mu$, we will immediately improve our results.}

\subsubsection{Accuracy of the Price Function.}

Forecasters are deterministic poly-time machines $\Fc$ that receive an input $t$, and output a number $q \in \cW_{\gamma}=\set{i \cdot \gamma: 0 \le i \le 1/\gamma} \subseteq [0,1]$.
Loosely speaking, we set up the price function so that the incentive of a forecaster $\Fc$ is to answer $q \in \cW_{\gamma}$ which is closest to $\Pr[X=1 \mid T=t]$.

A forecaster $\Fc$ partitions the set of possible $t$'s into $1/\gamma$ subsets $\set{\cB_q}_{q \in \cW_{\gamma}}$ for $\cB_q=\set{t:\Fc(t)=q}$. We will choose $\gamma$ to be a constant, $\gamma=\mu^{1/100}$, and set up the price function so that we can insure the following property:\footnote{The precise choice and properties of the price function comes up in other places in the argument, that we will not mention in this high level overview.}

\begin{description}
\item[\emph{Accuracy:}] If for a forecaster $\Fc$ there exists $q \in \cW_{\gamma}$ such that:
\begin{itemize}
\item $\Pr[T \in \cB_q] \ge \gamma^{10}$ (we will say that $\cB_q$ has significant weight. Note that the total weight of insignificant sets is $\gamma^{9}$ which we will neglect).
\item $q \ne \Pr[X=1\mid T \in \cB_q]$ (we will say that $\Fc$ errs on $\cB_q$).
\end{itemize}
\noindent
Then $\Fc$ can be improved by $\mu$, by simply ``correcting the error'' on $\cB_q$.
\end{description}

We  assume \wlg  that optimal forecasters self-correct their answers in the following sense: a poly-time forecaster $\Fc$ that receives $t$ and ``is about to'' output $q$, can sample many pairs $(X,T)$ by simulating the protocol $\Pi$  on his own. Once $\Fc$ obtained such a sample, it can:

\begin{itemize}
\item Check whether $\cB_q$ has significant weight.
\item If $\cB_q$ has significant weight, then  $\Fc$ can approximate $\Pr[X=1 \mid T \in \cB_q]$.
\item If this approximation $q'$ is far from $q$, then $\Fc$ discards $q$, and output the closest number to $q'$ in $\cW_{\gamma}$.
\end{itemize}
Applying self-correction cannot increase the price (except for exponentially small sampling errors).
Therefore, we can assume that $\mu$-optimal forecasters give accurate answers on significant weight $\cB_q$'s. (Note that for self-correcting we have to allow the forecaster to be randomized, but we ignore this technicality in this informal overview).

In the paper we also arrange another forecasting competition where the forecasters $\Fc(t)$ are required to predict $\Pr[Y=1\mid T=t,X=0]$ and $\Pr[Y=1\mid T=t,X=1]$. This competition is ``harder to control'' (as we need to carefully handle cases that $\Pr[X=0\mid T=t]$ or $\Pr[X=1\mid T=t]$ are very small). We do not describe this part, and only mention that using this competition we can show that: if for every set $\cB_q$ with significant weight $(X,Y\mid  T \in \cB_{q})$ are not correlated, then this will be reported by the winner of the second forecasting competition (that will report correctly that $\Pr[Y=1\mid T \in \cB_{q},X=0] \approx \Pr[Y=1\mid T \in \cB_{q},X=1]$, and that furthermore, this information can be used to decorrelize the protocol. (This part is quite technical, and we won't describe it in this section).

Therefore, from now on we can assume that either we were able to show that the protocol is uncorrelated (and won), or else, there exists $q'$ so that $\cB_{q'}$ has significant weight, and $\Pr[X=Y\mid T \in \cB_{q'}] \ge 1/2+a$ for some small constant $a$ that we control.

\subsection{A Win-Win Case-Analysis}

We will consider two cases, let $\lambda>0$ be a parameter, that we think of as a small constant. 
\begin{itemize}
\item There exists  $q'$ and set $\cB_{q'}$,  with $\lambda \le q' \le 1-\lambda$ and $\Pr[X=Y\mid T \in \cB_{q'}] \ge 1/2+a$.
\item For all sets $\cB_{q}$ of significant weight, it holds that  $q < \lambda$ or $q>1-\lambda$.
\end{itemize}

Let us first take care of the second case. We claim that in the second case the protocol is uncorrelated. Let us examine the second case. We can safely ignore all $q$'s such that $\cB_q$ does not have significant weight (as their total weight is small and they can be swallowed by the indistinguishability parameter $\rho$). For every $q$ where $\cB_q$ has significant weight, the forecaster $\Fc$ reports that $\Pr[X=1|T \in \cB_q]=q$ where $q$ is either $\lambda$-close to zero, or $\lambda$-close to one. By the accuracy property, this report is correct. This means that we can obtain
a decorelator $\Decr$ as follows: on input $t$, $\Decr$ computes $q=\Fc(t)$ and prepares the output $p_\Ac=q$.  Then, $\Decr$ uses random sampling (as explained before) to output an approximation $p_\Bc$ of $\Pr[Y=1\mid T \in \cB_q]$. (This can be done if $\cB_q$ has significant weight). Note that $\Decr$ indeed achieves a ``decorrelation'' of $\Pi$ (where the distinguishing parameter $\rho$ is slightly larger than $\gamma+\lambda$).

\subsection{Constructing Key Agreement}


We are left with the first case. We will show that in this case we can obtain a key-agreement. For that, it will be sufficient to achieve constant secrecy $s$ that is sufficiently smaller than the constant $a$ of the previous section. In order to develop intuition, we start with a simplifying assumption.

Suppose we are lucky and $q'=1/2$. Let us consider the following protocol $\sPi=(\sA,\sB)$. The two parties first engage in the protocol $\Pi=(\Ac,\Bc)$. Each of the parties $\sA,\sB$ runs $\Fc(T)$ on his own, and outputs the output that he receives in $\Pi$, if $\Fc(T) = 1/2$. Otherwise, if $\Fc(T) \ne 1/2$, then the party outputs a fresh random bit. Let us denote the outputs of this protocol by $\hat{X},\hat{Y}$ respectively.

We claim that this protocol has the secrecy property of a key agreement. For this, we note that if an adversary $\Ec(T)$ has $\Pr[\Ec(T)=\hat{X}] \ge 1/2+s$ then $\Pr[\Ec(T)=X\mid  T \in \cB_{1/2}] \ge 1/2+s$. This will imply that $\Fc$ can be improved by $\mu$ (contradicting the $\mu$-optimality of $\Fc$).

Loosely speaking, the latter statement follows because $\Fc$ could have used $\Ec$ to improve its forecasting on the set $\cB_{1/2}$: Clearly, the mere existence of $\Ec$ demonstrates that the value $1/2$ is an incorrect prediction in this set. Moreover, $\Ec$ splits the set $\cB_{1/2}$ into two sets $\cB_{1/2} \cap \set{t:\Ec(t)=0}$ and $\cB_{1/2} \cap \set{t:\Ec(t)=1}$, and $\Fc$ could have gained by using this information (that is available to $\Fc$ as $\Ec$ is poly-time). Specifically, $\Fc$ cans lightly decrease its prediction on the first set, and slightly increase its prediction on the second set. Such a modification is closer to the truth, and by the accuracy property it improves the price of $\Fc$.

\subsubsection{The One-Sided von-Neuman Protocol}

We are left with the case that $q' \ne 1/2$ and $q'$ is bounded away from zero and one. By accuracy, this means that $q' \approx \Pr[X=1\mid T \in \cB_{q'}]$. If we had the stronger ``information theoretic guarantee'' that for every $t \in \cB_{q'}$, $\Pr[X=1\mid T=t]=q'$, then we can use the von-Neuman extractor to convert the biassed coin $(X\mid T=t)$ into a fair coin. This inspires the following protocol:

The parties engage in two invocations of the original protocol $\Pi$; after these  invocations, party $\Ac$ holds $(X_1,X_2)$ and party $\Bc$ holds $(Y_1,Y_2)$. The transcript at this point is $(T_1,T_2)$. Party $\Ac$ checks whether $X_1\neq X_2$ and reports the answer to \Bc. Each party also checks whether $\Fc(T_1)=\Fc(T_2)$. If  answers to both questions are  positive,   party \Ac outputs $X_1$ and party \Bc outputs $Y_1$. Otherwise ($X_1= X_2$ or $\Fc(T_1)\neq \Fc(T_2)$), each party outputs a fresh random coin. By the existence of $q'$, the fact that we are in the first case, and the accuracy property, with constant probability it holds that $X_1 \ne X_2$ and $F(X_1)=F(X_2)=q'$. This is used to guarantee the agreement property of this protocol.

In the technical part we show that if the secrecy of this protocol is broken by an adversary $\Ec$, meaning that $\Ec$ predicts $X_1$ conditioned on the event $\set{X_1 \ne X_2,\Fc(T_1)=\Fc(T_2)}$, then $\Ec$ can be used to improve the forecaster $\Fc$ by $\mu$ (which is a contradiction to its $\mu$-optimality).
This argument follows the same lines as the case of $q'=1/2$ but is significantly more complicated.
